Repetita Iuvant: Data Repetition Allows SGD to Learn High-Dimensional Multi-Index Functions

Neural networks can identify low-dimensional relevant structures within high-dimensional noisy data, yet our mathematical understanding of how they do so remains scarce. Here, we investigate the training dynamics of two-layer shallow neural networks trained with gradient-based algorithms, and discuss how they learn pertinent features in multi-index models, that is target functions with low-dimensional relevant directions. In the high-dimensional regime, where the input dimension $d$ diverges, we show that a simple modification of the idealized single-pass gradient descent training scenario, where data can now be repeated or iterated upon twice, drastically improves its computational efficiency. In particular, it surpasses the limitations previously believed to be dictated by the Information and Leap exponents associated with the target function to be learned. Our results highlight the ability of networks to learn relevant structures from data alone without any pre-processing. More precisely, we show that (almost) all directions are learned with at most $O(d \log d)$ steps. Among the exceptions is a set of hard functions that includes sparse parities. In the presence of coupling between directions, however, these can be learned sequentially through a hierarchical mechanism that generalizes the notion of staircase functions. Our results are proven by a rigorous study of the evolution of the relevant statistics for high-dimensional dynamics.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We brake down our claim in the ones related to \emph{Single-Index models}, addressed in Section 3, and the ones for \emph{Multi-Index models}, addressed in Section~4.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The limitations of the setting are pointed out in the introduction, and in all relevant cited literature.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The statement and the assumptions are stated in the main paper, while the proofs are presented in detail in Appendix A.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the algorithms used for the simulation are described in the paper (and relevant cited literature). All plots are accompanied with description and parameters used.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code is provided through the repository linked in the main paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We detail the choice of the parameters in Main theorems and caption of Figures. We also provide Appendix~\ref{sec:app:implementation} with all the details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Every plot has error bars obtained by Gaussian average/std formula applied on many runs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experiments do not require any particular hardware and in principle can be run on any modern laptop.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We read the Code of Ethics and confirm that the paper is conform with it.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is a theoretical work with numerical illustrations; we do not foresee any potential societal impact.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not have safeguards because this is a theoretical work on simple architecture and data distribution.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We are the authors of the core part of the code and all the dependencies are used following their licenses.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code does not have a documentation, but is well commented. We believe it does not require any further explanation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This does not apply to our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This does not apply to our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/alternative.tex <==
\section{Conclusion, perspective and limitations}
We have pushed in this paper the  boundaries of learning multi-index models  in high-dimensional settings using gradient-type descent algorithms, and shown that, contrary to what was believed, they are very efficient in doing so. A natural direction would be to consider \cite{damian_2023_smoothing} to make them even closer to SQ bounds in the more difficult setting. While one limitation of our work is the asymptotic setting with Gaussian data, we note that numerical test shows that the prediction are already accurate, even at fairly moderate sizes. Additionally, a number of universality results shows that our scenario can be extend to more generic type of data (see e.g. \cite{montanari2022universality,pesce2023gaussian}). The next desirable step would be to look at structured data, learned by multi-layer network. This, however, represents a considerable challenge for current technics.

% \begin{wrapfigure}{R}{0.48\textwidth}
%            \includegraphics{figures/fig_exponential.pdf}{0.4\textwidth}
%             \caption{\textbf{Going beyond data resuing:} Exponential Loss (crosses) vs Square Loss (dots).}
%             \label{fig:exponential-lossH3}
% \end{wrapfigure}



% \begin{figure}
%     \centering
%     \includegraphics[height=0.24\textwidth]{figures/fig_exponential.pdf}
% i    \caption{\textbf{Going beyond data resuing:} Exponential Loss (crosses) vs Square Loss (dots).}
%     \label{fig:exponential-lossH3}
% \end{figure}

==> sections_old/alternative.tex <==
\section{Conclusion, perspective and limitations}
We have pushed in this paper the  boundaries of learning multi-index models  in high-dimensional settings using gradient-type descent algorithms, and shown that, contrary to what was believed, they are very efficient in doing so. A natural direction would be to consider \cite{damian_2023_smoothing} to make them even closer to SQ bounds in the more difficult setting. While one limitation of our work is the asymptotic setting with Gaussian data, we note that numerical test shows that the prediction are already accurate, even at fairly moderate sizes. Additionally, a number of universality results shows that our scenario can be extend to more generic type of data (see e.g. \cite{montanari2022universality,pesce2023gaussian}). The next desirable step would be to look at structured data, learned by multi-layer network. This, however, represents a considerable challenge for current technics.

% \begin{wrapfigure}{R}{0.48\textwidth}
%            \includegraphics{figures/fig_exponential.pdf}{0.4\textwidth}
%             \caption{\textbf{Going beyond data resuing:} Exponential Loss (crosses) vs Square Loss (dots).}
%             \label{fig:exponential-lossH3}
% \end{wrapfigure}



% \begin{figure}
%     \centering
%     \includegraphics[height=0.24\textwidth]{figures/fig_exponential.pdf}
% i    \caption{\textbf{Going beyond data resuing:} Exponential Loss (crosses) vs Square Loss (dots).}
%     \label{fig:exponential-lossH3}
% \end{figure}

==> sections_old/intro.tex <==
\section{Introduction}
Gradient Descent-based algorithms such as  Stochastic Gradient Descent (SGD) and its variations, are a fundamental tool in training neural networks, and are therefore the subject of intense theoretical scrutiny. Recent years have witnessed significant advancements in understanding their dynamics and the learning mechanisms of neural nets. Significant progress has been made, in particular, in the case of two-layer networks thanks, in part, to the so-called mean-field analysis \citep{mei2018mean,chizat2018global,rotskoff2018trainability,sirignano2020mean}). A large part of the theoretical approach focused on {\it one-pass} optimization algorithms, where {\it each iteration involves a new fresh batch of data}. In particular, in the mathematically solvable case of  high-dimensional synthetic Gaussian data, and a low dimensional a multi-index target function model, the class of functions efficiently learned by these \textit{one-pass} methods has been thoroughly analyzed in a series of recent works, and have been shown to be limited by the so-called information exponent \citep{BenArous2021} and leap exponent \citep{abbe2022merged, abbe2023sgd}. These analyses have sparked many follow-up theoretical works over the last few months, see, e.g. \cite{damian2022neural,damian_2023_smoothing,dandi2023twolayer,bietti2023learning,ba2023learning, moniri2023theory, mousavihosseini2023gradientbased,zweig2023symmetric}, leading to a picture where SGD dynamics is governed by the information exponent, that is, the order of the first non-zero Hermite coefficient of the target.

A common point between all these works, however, is that they considered the idealized situation where one process data one sample at a time, all of them independently identically distributed, without any repetition. This is, however, not a realistic situation in practice. Indeed, most datasets contains similar data-points, so that repetition occurs (see e.g. for repetition and duplicate in CIFAR \citep{barz2020we}) Additionally, it is common in machine learning to  repeatedly go through the same mini-batch of data multiple time over epoch. Finally, many gradient algorithms, often used in machine learning in Lookahead optimizers \citep{lookahead}, Extragradient methods \citep{Korpelevich1976TheEM}, or Sharpness Aware Minimization (SAM) \citep{foret2021sharpnessaware}, are {\it explicitly} few gradient steps over the exact same data-point. It is thus natural to wonder if using such extra-gradient algorithms, or simply reusing many time some data, would change the picture with respect to the current consensus.


There are good reason to believe this to be the case. Indeed, it has been observed very recently \citep{dandi2024benefits} that iterating twice over large ($O(d)$) datasets was enough to alter the picture reached in 
\cite{BenArous2021,abbe2022merged, abbe2023sgd}. Indeed \cite{dandi2024benefits} showed that their exist functions that can be learned over few (just two) batch repetition, while they require a much larger (i.e. polynomial in $d$) number of steps otherwise.
%gradient descent when repeating over data batches {\it surpasses} (that scale linearly with the input dimension) the limitations imposed by the information and leap exponents, achieving a positive correlation with the target function for a much broader class than the staircase functions \cite{abbe2021staircase}. 
While the set of function considered in this work was limited, the conclusion is indeed surprising, thus motivating the following question: 
\begin{center}
\textit{
Can data repetition increase the efficiency of SGD when learning any multi-index functions?
% Is there a fundamental gap of processing data online with respect to repeating larger batches? \\
% Are single-pass algorithms intrinsically sub-efficient with respect to the multiple-pass one?
} 
\end{center}

% {\bf the point is that the SGD ideal situation is not realistic and very fragile, and Dandi et al already show tojs in a very specific setting (O(1)) easy function, two iterations and O(D) batched reusined) Our point is to study what happens in  more generic siutation bla bla blabl argue for our setting... (i) proxy ofr realistic sutaiton where data or correlated data are reused, and (ii) in pratice people are foten using SAM, look head, federated learning...}

We establish a positive answer to the above question by the analysis of more realistic optimization schemes with respect to the standard One-Pass SGD. Indeed, the hardness exponents developed in the seminal works \cite{abbe2021staircase, BenArous2021} are substantially bound to the idealized training scenario that considers i.i.d data. Slight modifications to this training scenario toward a more realistic setting starkly change the global picture. Such slight modifications include: a) non-vanishing correlations between different data points, that is a natural requirement for real datasets; b) processing the same data point multiple times in the optimization routine, i.e., a standard step in any algorithmic procedure when looping over different epochs. 

We consider an analytically tractable a single-pass training scheme to model these changes: we process one Gaussian sample at a time, but {\it the gradient step is repeated twice}! This simple adjustment 
to the idealized SGD optimization scheme, which is actually often used in machine learning in Lookahead optimizers \citep{lookahead}, Extragradient methods \citep{Korpelevich1976TheEM}, or in the context of Sharpness Aware Minimization (SAM \cite{foret2021sharpnessaware}), will be seen to make single-pass algorithms drastically more efficient, and, as we will see, as efficient than our best algorithms in most cases. \looseness=-1

We show in particular that most multi-index function are learned with total sample complexity either $O(d)$ or $O(d \log d)$ if they are related to the presence of a symmetry, without any need for preprocessing of the data that is performed in various works (See e.g., \cite{mondelli2018fundamental,luo2019optimal,maillard2020phase,chen2020learning}).  Our results thus demonstrate that shallow neural networks turns out to be significantly more powerful than previously believed \citep{BenArous2021,abbe2022merged,abbe2023sgd,arnaboldi.stephan.ea_2023_high} in identifying relevant feature in the data. In fact, they are shown in many (but not all) cases to saturate the bounds predicted by statistical queries (SQ)  \citep{damian2024computational} (rather than the more limited correlation statistical queries (CSQ) bounds that were characteristic of the former consensus \citep{BenArous2021,abbe2023sgd}). Our conclusions follow from the rigorous analysis of the overlaps between the trained weight vectors with the low-dimensional relevant subspace that draws inspiration from the pivotal works of \cite{saad.solla_1995_line, PhysRevE.62.5444,A.C.C.Coolen_2000,BenArous2021}.



==> sections_old/multi_index.tex <==
\section{Multi-Index Model}
We now investigate the superiority of Algorithm~\ref{algo:optimizer_main_step} over the idealized One-Pass SGD training scheme when learning multi-index targets. In this setting, the networks weights can align with only a few select directions from $V^\star$. To quantify this behavior, we define directional versions of the Information and Generative Exponents:
\begin{definition}\label{def:ie_ge_multi}
    Let $\vec{v}\in V^\star$. The Information Exponent $\ell_{\vec{v}}$ (resp. Generative exponent $\ell^\star_{\vec{v}}$) of $y$ in the direction $\vec v$ is the smallest $k$ such that
    \[ \Ea{yH_k(\langle \vec{v}, \vec{z} \rangle)} \neq 0 \quad (\text{resp.} \  \Ea{f_{\vec{v}}(y)H_k(\langle \vec{v}, \vec{z} \rangle)} \neq 0 ) \]
    for a function $f_{\vec{v}}$. We also let $\ell = \min_{\vec{v}}\ell_{\vec{v}}$ and $\ell^\star = \min_{\vec{v}}\ell^\star_{\vec{v}}$.
\end{definition}
The identification of the class of hard functions has been subject of intense theoretical scrutiny \citep{abbe2021staircase,abbe2022merged,abbe2023sgd,dandi2023twolayer,bietti2023learning}; and for the problem of initial alignment it was shown to depend on the Information exponent defined above. 
Thus, similarly to the single-index scenario, the time complexity needed for Algorithm~\ref{algo:optimizer_main_step} to weakly recover the target subspace follows the law in eq.~\eqref{eq:gba_time_scaling} for the multi-index information exponent $\ell$. A natural question is thus to ask whether the class of Algorithm~\ref{algo:optimizer_main_step} also allows us to bypass this requirement. We show that this is indeed the case. Consider a neural network as in Equation~\eqref{eq:def_nn}; we modify the assumptions of Theorem~\ref{thm:single_index_recovery} as follows:
\begin{assumptionp}{\ref*{assump:spherical_corr}'}
    We run the spherical version of Algorithm~\ref{algo:optimizer_main_step}, with different $\rho_j \sim \mathrm{Unif}\{\pm1\}$ for each neuron $j$.    
\end{assumptionp}

\begin{assumptionp}{\ref*{assump:init}'}
    All initial vectors $\vec{w}_{0, j}$ are drawn i.i.d with $\vec{w}_{0, j} \sim \mathrm{Unif}(\mathbb{S}^{d-1})$. The initial values for the second layer are drawn according to $a_{j, 0} \sim \mathrm{Unif}([-1, 1])$.
\end{assumptionp}

\begin{theorem}
    Let $U^\star \subseteq V^\star$ be the span of all vectors $\vec{v}$ with $\ell_{\vec{v}}^\star = \ell^\star$, and $\delta > 0$. There exists constants $\gamma_0(\delta), C(\delta)$ depending only on $\delta$ such that if we take $p \geq C(\delta)k$ and
    \begin{itemize}
        \item if $\ell_p^\star = 1$, $\gamma = \gamma_0(\delta) d^{-1}$ and $T = C(\delta)d$,
        \item if $\ell_p^\star = 2$, $\gamma = \gamma_0(\delta) (d\log(d))^{-1}$ and $T = C(\delta)d\log(d)^2$,
    \end{itemize}
    then the following holds. With probability $1 - \delta$, there exists a $t \leq T$ such that
    \begin{itemize}
        \item at least a positive proportion of the vectors $\vec{w}_{t, i}$ satisfy $\norm{\Pi^\star \vec{w}_{t, i}} \geq \eta$,
        \item the vectors $(\Pi^\star \vec{w}_{t, i})_{i \in[p]}$ span $U^\star$.
    \end{itemize}
\end{theorem}

\textcolor{purple}{{\bf THEOREM 4: Sketch of proof:}  Using the formulas of [2,3]: writing $\mathbf{p}_t$ the projection of $\mathbf{w}_t$ on $V^\star$, the approximate difference equations for $\mathbf{p}_t$ in the case where $\ell_p^\star = 1$ (resp. $\ell_p^\star = 2$) read $\mathbf{p}_{t+1} = \mathbf{p}_t + \gamma \mathbf{v}^\star$ (resp. $\mathbf{p}_{t+1} = \mathbf{p}_t + \gamma A^\star \mathbf{p}_t$). In both cases, those dynamics can be translated to one-dimensional ones by considering $\langle \mathbf{v}, \mathbf{p}_t \rangle$ for either $\mathbf{v} = \mathbf{v}^\star$ or $\mathbf{v}$ an eigenvector of $A^\star$. }


Our simulations enable us to affirmatively answer this question. We illustrate this numerically by comparing the performance of One-Pass SGD with Algorithm~\ref{algo:optimizer_main_step} in Figure~\ref{fig:main:multi_index_complete}; we show that the dynamics of the latter algorithm is governed by the multi-index Generative Exponent (Def.~\ref{def:ie_ge_multi}).

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[height=0.95\textwidth, trim={0 8 0 0}, clip]{figures/fig2_k1_kstar1.pdf}
        \caption{$h^\star(x_1,x_2)=x_1+x_1x_2$}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[height=0.95\textwidth, trim={0 8 0 0}, clip]{figures/fig2_k2_kstar2.pdf}
    \caption{$h^\star(x_1,x_2)=\mathrm{sign}{(x_1x_2)}$}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[height=0.95\textwidth, trim={0 8 0 0}, clip]{figures/fig2_k3_kstar1.pdf}
    \caption{$h^\star(x_1,x_2)=x_1+\mathrm{He}_3(x_2)$}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[height=0.95\textwidth, trim={0 8 0 0}, clip]{figures/fig2_k3_kstar2.pdf}
    \caption{$h^\star(x_1,x_2,x_3)=x_1x_2x_3$}
    \end{subfigure}

    \caption{\textbf{Learning multi-index targets --}
    Evolution of the maximum Cosine Similarities attained by EgD (crosses) and SGD (dots) as a function of the normalized iteration time. Different target directions $\{\vec w^\star_r\}_{r \in [k]}$ are identified by different colors: $\vec w^\star_1$ (blue), $\vec w^\star_2$ (orange), $\vec w^\star_3$ (green).
    The dashed horizontal line $\frac{1}{\sqrt{d}}$ is a visual guide to place random performance. See details in App.~\ref{sec:app:implementation}
    \textbf{(a)~$(\ell,\ell^\star)=(1,1)$:} both the algorithm learn the first direction in linear time, and they also learn the second in another \(O(d)\) steps using the staircase mechanism.
    \textbf{(b) $(\ell,\ell^\star)=(2,2)$:} both the algorithm learn the two direction simultaniously in \(O(d\log d)\) steps.
    \textbf{(c)~$(\ell_{\vec w^\star_2},\ell_{\vec w^\star_2}^\star)=(3,1)$:} both the algorithms learn \(\vec w^\star_1\) in linear time, but only EgD can also learn \(\vec w^\star_2\) in \(O(d)\); SGD requires \(O(d^2)\) steps to learn \(\vec w^\star_2\).
    \textbf{(d) $(\ell,\ell^\star)=(3,2)$:} EgD learns all the 3 directions simultaneously in \(O(d\log d)\) steps, while SGD needs quadratic time to achieve the same recovery. 
    }
    \label{fig:main:multi_index_complete}
\end{figure}

\subsection{Numerical investigation with multi-index target}\label{subsec:multi_numerics}

% (\lp{Def.~\ref{def:hardness_subspace}}). 
We measure the maximal cosine similarity between the hidden layer neurons and the different rows of the target's weight matrix $W^\star$ as a function of the iteration time. We set without loss of generality the target's directions to the standard basis of $\mathbb{R}^d$ to ease the notation. The algorithms considered are again EgD and vanilla One-Pass SGD. We again refer to Appendix \ref{sec:app:implementation} for the implementation details.

\textbf{SGD-easy non-symmetric targets ($\ell \!=\! \ell^\star \!=\! 1$) --} Fig.~\ref{fig:main:multi_index_complete}, left, shows $h^\star(x_1,x_2) = x_1 + x_1x_2$. Here both SGD and Alg.~\ref{algo:optimizer_main_step} learn in $T= O(d)$ the directions $(\vec w^\star_1, \vec w^\star_2)$.

\textbf{SGD-easy symmetric targets ($\ell \!=\! \ell^\star \!=\! 2$) --} Fig.~\ref{fig:main:multi_index_complete}, center left, shows $h^\star(x_1,x_2) = x_1x_2$.  Here both SGD and Alg.~\ref{algo:optimizer_main_step} learn in $T=O(d \log d)$ the directions $(\vec w^\star_1, \vec w^\star_2)$. 

\textbf{Non-symmetric targets with SGD-easy and hard directions ($\ell_{\vec{v}} > 2, \ell^\star_{\vec{v}}=1$) --} Fig.~\ref{fig:main:multi_index_complete}, center-right, shows $h^\star(x_1,x_2) \!=\! x_1 \!+\! \mathrm{He}_3(x_2) $. Here both SGD and Alg.~\ref{algo:optimizer_main_step} learn in $T=O(d)$ the direction $\vec w^\star_1$, that satisfies $\ell_{\vec{w_1^\star}} = \ell_{\vec{w_1}^\star}^\star = 1$. However, since $\ell_{\vec{w_2^\star}} = 3$ while $\ell_{\vec{w_2^\star}}^\star = 1$, One-Pass SGD suffers from the limitations detailed in eq.~\eqref{eq:gba_time_scaling} and requires $\Omega(d^2)$ samples to learn the second direction $\vec w^\star_2$, . This contrasts with the behaviour of Alg.~\ref{algo:optimizer_main_step} that learns also $\vec w^\star_2$ in $T=O(d)$ steps.

\textbf{SGD-hard symmetric targets ($\ell > 2,  \ell^\star =2$) --} The right section Fig.~\ref{fig:main:multi_index_complete} shows $h^\star(x_1,x_2,x_3) = x_1 x_2 x_3$. The Information Exponent is $\ell=3$ and hence vanilla SGD is not able to learn any direction in the target subspace in $T=O(d \log d)$ iterations. However, Algorithms~\ref{algo:optimizer_main_step} learns in $T=O(d \log d)$ steps all the three directions $\{\vec w^\star_1, \vec w^\star_2, \vec w^\star_3\}$ since the Generative Exponents $\ell_{\vec{w}^\star_r}^\star$ are all equal to two.

\subsection{Learning hard functions through a hierarchical mechanism}\label{subsec:staircase}


% \color[purple]{THEOREM ASSUMING LEARNED DIRECTION...}

The investigation of the hierarchical nature of SGD learning has attracted noticeable attention \citep{abbe2021staircase,abbe2022merged,abbe2023sgd, dandi2023twolayer}. In this paper, we portray a completely different picture in terms of computational efficiencies when data repetition is considered in the algorithmic SGD routine. One may wonder if there is a generalization of such a hierarchical learning mechanism to the present novel setting; we show that coupling between directions can hierarchically guide the learning process. 


The Left panel in Fig.~\ref{fig:main:staircase1} shows an example of the so-called staircase functions \citep{abbe2021staircase}, i.e. $f^\star(\vec z) = z_1 + z_1 \mathrm{He}_3(z_2)$. While one-pass SGD needs to learn hierarchically first the direction $\vec w^\star_1$ in $T=O(d)$ and then $\vec w^\star_2$ in $T=O(d^2)$, Algorithm~\ref{algo:optimizer_main_step} easily learns both in linear time. This observation could lead to infer that hierarchical learning mechanisms are not present when more realistic training scenarios are considered.

\begin{figure}
    % \begin{center}
        \begin{subfigure}[t]{0.24\textwidth}
        \centering
            \includegraphics[height=0.95\textwidth, trim={0 8 0 0}, clip]{figures/fig2_k3_kstar1_staircase.pdf}
            \caption{$f^\star(\vec z)= z_1 + z_1 \mathrm{He}_3(z_2)$}
        \end{subfigure}    
        \hspace{.5cm}
        \begin{subfigure}[t]{0.74\textwidth}
            \centering
            \includegraphics[height=0.31\textwidth, trim={0 8 0 0}, clip]{figures/figs_SQStair_long.pdf}
            \caption{$f_{\mathrm{sign}}^\star(\vec{z}) = \mathrm{sign}(z_1z_2z_3), \quad f^\star_{\mathrm{stair}}(\vec z) = \mathrm{He}_2(z_1) + \mathrm{sign}(z_1z_2z_3)$}
        \end{subfigure}    
    % \end{center}
\caption{
    \textbf{Hierarchical picture of learning --} Evolution of the maximum Cosine Similarities with different target directions $\{\vec w^\star_r\}_{r \in [k]}$ are identified by different colors: $\vec w^\star_1$ (blue), $\vec w^\star_2$ (orange), $\vec w^\star_3$ (green) as a function of the normalized iteration time.
    \textbf{(a):} both the algorithms learn \(\vec w^\star_1\) in linear time, but only EgD can also learn \(\vec w^\star_2\) in \(O(d)\) using staircase mechanism; SGD requires another \(O(d^2)\) steps to take advatage of the staircase and learn \(\vec w^\star_2\).
    \textbf{(b):} EgD performance for the target function $f^\star_{\mathrm{stair}}$ (dots) and $f^\star_{\mathrm{sign}}$(squares); we plot in separate subplots the overlap with different directions to highlight the presence of hierarchical learning mechanism. Learning the first target direction $\vec w^\star_1$ triggers the hierarchical mechanism and EgD is able to weakly recover the full target subspace $\mathrm{Span}(\vec w^\star_1, \vec w^\star_2, \vec w^\star_3)$ in $O(d \log d)$, while this does not happen when removing \(\mathrm{He}_2(x_1)\) from the target.
    See App.~\ref{sec:app:implementation} for additional details.}
    % \includegraphics[height=0.27\textwidth]{figures/fig2_k3_kstar1_staircase.pdf}
\label{fig:main:staircase1}
\end{figure}

To refute this, we illustrate in the right panel of Fig.~\ref{fig:main:staircase1} a scenario that precisely exemplifies the presence of hierarchical mechanisms within Algorithm~\ref{algo:optimizer_main_step}. We run this algorithm on two different target functions, $f_{\mathrm{sign}}^\star(\vec{z}) = \mathrm{sign}(z_1z_2z_3)$ and $f^\star_{\mathrm{stair}}(\vec z) = \mathrm{He}_2(z_1) + \mathrm{sign}(z_1z_2z_3)$. We show in App. \ref{sec:app:proofs} that $3-$sparse parities of the form $\mathrm{sign}(z_1z_2z_3)$ are hard functions even for SGD with data repetition (Algorithm~\ref{algo:optimizer_main_step}), and indeed they are not learned in (almost) linear time. On the other hand, for the function $f^\star_{\mathrm{stair}}$, our simulations predict that the first direction $\vec w^\star_1$ is learned in $T = O(d \log d)$ iterations (see the rightmost panel of Fig.~\ref{fig:main:multi_index_complete}). However, once the direction $\vec w^\star_1$ is learned, it can be used to obtain order-one correlation with $\{\vec w^\star_2, \vec w^\star_3\}$ again in $T = O(d \log d)$ steps. While the latter example belongs to the class of ``CSQ'' staircase function depicted in \cite{abbe2021staircase}, novel ``SQ'' hierarchical mechanisms arise in our framework, such as for instance the function $f_{\rm sq-stair}^\star(\vec z) = \mathrm{He}_4(z_1) + \mathrm{sign}(z_1z_2z_3)$ (see Fig.~\ref{fig:main:staircase2}). 

\begin{figure}
    \centering
    \includegraphics[width=.6\textwidth]{figures/figs_SQStairH4_long.pdf}
    \caption{\textbf{Novel hierarchical picture of learning --} Evolution of the maximum Cosine Similarities attained by EgD with different target directions $\{\vec w^\star_r\}_{r \in [k]}$ are identified by different colors: $\vec w^\star_1$ (blue), $\vec w^\star_2$ (orange), $\vec w^\star_3$ (green) as a function of the normalized iteration time. The target function is $f^\star_{\rm sq-stair}(\vec z)= \mathrm{He}_4(z_1) + \mathrm{sign}(z_1z_2z_3)$, that is an SQ-staircase, but not a CSQ-staircase. EgD learn $\vec w^\star_1$ in \(O(d\log d)\) steps and use the information to learn the other two directions in another \(O(d\log d)\) steps. SGD (not showed in the plot) cannot take advantage of the staircas mechanism since $\mathrm{He}_4(z_1)$ and $\mathrm{sign}(z_1z_2z_3)$ have information exponent \(\ell = 4\) and \(\ell = 3\) respectively. See App.~\ref{sec:app:implementation} for additional details.}
    \label{fig:main:staircase2}
    
\end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=.6\textwidth]{figures/figs_SQStairH4_long.pdf}
%     \caption{learning dynamic of the three hidden direction of the SQ-staircase function \(h^\star(\vec z) = \mathrm{He}_4(z_1) + 5\mathrm{sign}(z_1z_2z_3)\), that is not CSQ-staircase. \(\gamma_0=0.01\), \(\rho_0=0.1\), \(d=1024\), \(\sigma = \mathrm{ReLU}\). See details in App.~\ref{sec:app:implementation}}
%     \label{fig:app:sq-staircase}
% \end{figure}



==> sections_old/sections/alternative.tex <==
\section{Conclusion, perspective and limitations}
We have pushed in this paper the  boundaries of learning multi-index models  in high-dimensional settings using gradient-type descent algorithms, and shown that, contrary to what was believed, they are very efficient in doing so. A natural direction would be to consider \cite{damian_2023_smoothing} to make them even closer to SQ bounds in the more difficult setting. While one limitation of our work is the asymptotic setting with Gaussian data, we note that numerical test shows that the prediction are already accurate, even at fairly moderate sizes. Additionally, a number of universality results shows that our scenario can be extend to more generic type of data (see e.g. \cite{montanari2022universality,pesce2023gaussian}). The next desirable step would be to look at structured data, learned by multi-layer network. This, however, represents a considerable challenge for current technics.

% \begin{wrapfigure}{R}{0.48\textwidth}
%            \includegraphics{figures/fig_exponential.pdf}{0.4\textwidth}
%             \caption{\textbf{Going beyond data resuing:} Exponential Loss (crosses) vs Square Loss (dots).}
%             \label{fig:exponential-lossH3}
% \end{wrapfigure}



% \begin{figure}
%     \centering
%     \includegraphics[height=0.24\textwidth]{figures/fig_exponential.pdf}
% i    \caption{\textbf{Going beyond data resuing:} Exponential Loss (crosses) vs Square Loss (dots).}
%     \label{fig:exponential-lossH3}
% \end{figure}

==> sections_old/sections/intro.tex <==
\section{Introduction}
Gradient Descent-based algorithms such as  Stochastic Gradient Descent (SGD) and its variations, are a fundamental tool in training neural networks, and are therefore the subject of intense theoretical scrutiny. Recent years have witnessed significant advancements in understanding their dynamics and the learning mechanisms of neural nets. Significant progress has been made, in particular, in the case of two-layer networks thanks, in part, to the so-called mean-field analysis \citep{mei2018mean,chizat2018global,rotskoff2018trainability,sirignano2020mean}). A large part of the theoretical approach focused on \emph{one-pass} optimization algorithms, where \emph{each iteration involves a new fresh batch of data}. In particular, in the mathematically solvable case of  high-dimensional synthetic Gaussian data, and a low dimensional a multi-index target function model, the class of functions efficiently learned by these \textit{one-pass} methods has been thoroughly analyzed in a series of recent works, and have been shown to be limited by the so-called information exponent \citep{BenArous2021} and leap exponent \citep{abbe2022merged, abbe2023sgd}. These analyses have sparked many follow-up theoretical works over the last few months, see, e.g. \cite{damian2022neural,damian_2023_smoothing,dandi2023twolayer,bietti2023learning,ba2023learning, moniri2023theory, mousavihosseini2023gradientbased,zweig2023symmetric}, leading to a picture where SGD dynamics is governed by the information exponent, that is, the order of the first non-zero Hermite coefficient of the target.

A common point between all these works, however, is that they considered the idealized situation where one process data one sample at a time, all of them independently identically distributed, without any repetition. This is, however, not a realistic situation in practice. Indeed, most datasets contains similar data-points, so that repetition occurs (see e.g. for repetition and duplicate in CIFAR \citep{barz2020we}) Additionally, it is common in machine learning to  repeatedly go through the same mini-batch of data multiple time over epoch. Finally, many gradient algorithms, often used in machine learning in Lookahead optimizers \citep{lookahead}, Extragradient methods \citep{Korpelevich1976TheEM}, or Sharpness Aware Minimization (SAM) \citep{foret2021sharpnessaware}, are \emph{explicitly} few gradient steps over the exact same data-point. It is thus natural to wonder if using such extra-gradient algorithms, or simply reusing many time some data, would change the picture with respect to the current consensus.


There are good reason to believe this to be the case. Indeed, it has been observed very recently \citep{dandi2024benefits} that iterating twice over large ($O(d)$) datasets was enough to alter the picture reached in 
\cite{BenArous2021,abbe2022merged, abbe2023sgd}. Indeed \cite{dandi2024benefits} showed that their exist functions that can be learned over few (just two) batch repetition, while they require a much larger (i.e. polynomial in $d$) number of steps otherwise.
%gradient descent when repeating over data batches \emph{surpasses} (that scale linearly with the input dimension) the limitations imposed by the information and leap exponents, achieving a positive correlation with the target function for a much broader class than the staircase functions \cite{abbe2021staircase}. 
While the set of function considered in this work was limited, the conclusion is indeed surprising, thus motivating the following question: 
\begin{center}
\textit{
Can data repetition increase the efficiency of SGD when learning any multi-index functions?
% Is there a fundamental gap of processing data online with respect to repeating larger batches? \\
% Are single-pass algorithms intrinsically sub-efficient with respect to the multiple-pass one?
} 
\end{center}

% {\bf the point is that the SGD ideal situation is not realistic and very fragile, and Dandi et al already show tojs in a very specific setting (O(1)) easy function, two iterations and O(D) batched reusined) Our point is to study what happens in  more generic siutation bla bla blabl argue for our setting... (i) proxy ofr realistic sutaiton where data or correlated data are reused, and (ii) in pratice people are foten using SAM, look head, federated learning...}

We establish a positive answer to the above question by the analysis of more realistic optimization schemes with respect to the standard One-Pass SGD. Indeed, the hardness exponents developed in the seminal works \cite{abbe2021staircase, BenArous2021} are substantially bound to the idealized training scenario that considers i.i.d data. Slight modifications to this training scenario toward a more realistic setting starkly change the global picture. Such slight modifications include: a) non-vanishing correlations between different data points, that is a natural requirement for real datasets; b) processing the same data point multiple times in the optimization routine, i.e., a standard step in any algorithmic procedure when looping over different epochs. 

We consider a simple yet analytically tractable single-pass training scheme: processing one Gaussian sample at a time, but \emph{repeating the gradient step twice}. This minor adjustment, common in Lookahead optimizers \citep{lookahead}, Extragradient methods \citep{Korpelevich1976TheEM}, and Sharpness-Aware Minimization (SAM) \citep{foret2021sharpnessaware}, significantly boosts efficiency. In fact, we will see that this approach matches the performance of our best algorithms in most cases.

We show in particular that most multi-index function are learned with total sample complexity either $O(d)$ or $O(d \log d)$ if they are related to the presence of a symmetry, without any need for preprocessing of the data that is performed in various works (See e.g., \cite{mondelli2018fundamental,luo2019optimal,maillard2020phase,chen2020learning}).  Our results thus demonstrate that shallow neural networks turns out to be significantly more powerful than previously believed \citep{BenArous2021,abbe2022merged,abbe2023sgd,arnaboldi.stephan.ea_2023_high} in identifying relevant feature in the data. In fact, they are shown in many (but not all) cases to saturate the bounds predicted by statistical queries (SQ)  \citep{damian2024computational} (rather than the more limited correlation statistical queries (CSQ) bounds that were characteristic of the former consensus \citep{BenArous2021,abbe2023sgd}). Equivalently, it roughly  mirrors the prediction of the approximate message passing analysis in \citep{troiani2024fundamental}. Our conclusions follow from the rigorous analysis of the overlaps between the trained weight vectors with the low-dimensional relevant subspace that draws inspiration from the pivotal works of \cite{saad.solla_1995_line, PhysRevE.62.5444,A.C.C.Coolen_2000,BenArous2021}.

Concurrently with the present work, \citep{lee2024neural} also studies the properties of SGD under data repetition in neural networks. We discuss the differences between our works in Section~\ref{subsec:single_index_discussion}.



==> sections_old/sections/multi_index.tex <==
\begin{figure}[t]
    \centering
    \subfigure[{$\scriptstyle h^\star(\vec x) = x_1+x_1x_2$}]{%
        \includegraphics[height=0.22\textwidth, trim={0 8 0 0}, clip]{figures/fig2_k1_kstar1.pdf}
        \label{fig:multi_index_1}
    }\hfill
    \subfigure[{$\scriptstyle h^\star(\vec x) = \mathrm{sign}{(x_1x_2)}$}]{%
        \includegraphics[height=0.22\textwidth, trim={0 8 0 0}, clip]{figures/fig2_k2_kstar2.pdf}
        \label{fig:multi_index_2}
    }\hfill
    \subfigure[{$\scriptstyle h^\star(\vec x) = x_1+\mathrm{He}_3(x_2)$}]{%
        \includegraphics[height=0.22\textwidth, trim={0 8 0 0}, clip]{figures/fig2_k3_kstar1.pdf}
        \label{fig:multi_index_3}
    }\hfill
    \subfigure[{$\scriptstyle h^\star (\vec x) = x_1x_2x_3$}]{%
        \includegraphics[height=0.22\textwidth, trim={0 8 0 0}, clip]{figures/fig2_k3_kstar2.pdf}
        \label{fig:multi_index_4}
    }

    \caption{\textbf{Learning multi-index targets --}
    Evolution of the maximum Cosine Similarities attained by EgD (crosses) and SGD (dots) as a function of the normalized iteration time. The Different directions $\{\vec w^\star_r\}_{r \in [k]}$ are identified by colors: $\vec w^\star_1$ (blue), $\vec w^\star_2$ (orange), $\vec w^\star_3$ (green).
     (dashed horizontal line $\frac{1}{\sqrt{d}}$ is a visual guide to place random performance). 
    \textbf{(a)~$(\ell,\ell^\star)=(1,1)$:} both  algorithms learn the first direction in linear time, as well the second one in $O(d)$ steps using the staircase mechanism.
    \textbf{(b) $(\ell,\ell^\star)=(2,2)$:} both  algorithms learn the two directions simultaneously in $O(d\log d)$ steps.
    \textbf{(c)~$(\ell_{\vec w^\star_2},\ell_{\vec w^\star_2}^\star)=(3,1)$:} both algorithms learn $\vec w^\star_1$ in linear time, but only EgD learns $\vec w^\star_2$ in $O(d)$; SGD instead requires $O(d^2)$.
    \textbf{(d) $(\ell,\ell^\star)=(3,2)$:} EgD learns all 3 directions simultaneously in $O(d\log d)$ steps, while SGD needs $O(d^2)$ time.  (Details in App.~\ref{sec:app:implementation}).}
    \label{fig:main:multi_index_complete}
\end{figure}

\section{Multi-Index Model}
We now investigate the superiority of Algorithm~\ref{algo:optimizer_main_step} over the idealized One-Pass SGD training scheme when learning multi-index targets. In this setting, the networks weights can align with only a few select directions from $V^\star$. To quantify this behavior, we define directional versions of the Information and Generative Exponents (see also \citep{troiani2024fundamental}):
\begin{definition}\label{def:ie_pge_multi}
    Let $\vec{v}\in V^\star$. The Information Exponent $\ell_{\vec{v}}$ (resp. Polynomial Generative Exponent $\ell^\star_{\vec{v}}$) of $y$ in the direction $\vec v$ is the smallest $k$ such that
    \[ \Ea{yH_k(\langle \vec{v}, \vec{z} \rangle)} \neq 0 \quad (\text{resp.} \  \Ea{p_{\vec{v}}(y)H_k(\langle \vec{v}, \vec{z} \rangle)} \neq 0 ) \]
    for a polynomial $p_{\vec{v}}$. We also let $\ell = \min_{\vec{v}}\ell_{\vec{v}}$ and $\ell_p^\star = \min_{\vec{v}}\ell^\star_{\vec{v}}$.  The minimal subspace $U^\star \subseteq V^\star$ is defined as the smallest subspace $U$ such that $\ell_\vec{v} > \ell$ (resp. $\ell_{\vec{v}}^\star > \ell_p^\star$) for every $v\in U^\bot$.
\end{definition}
The identification of the class of hard functions has been subject of intense theoretical scrutiny \citep{abbe2021staircase,abbe2022merged,abbe2023sgd,dandi2023twolayer,bietti2023learning,troiani2024fundamental}; and for the problem of initial alignment it was shown to depend on the Information exponent defined above. 
Thus, similarly to the single-index scenario, the time complexity needed for Algorithm~\ref{algo:optimizer_main_step} to weakly recover the target subspace follows the law in eq.~\eqref{eq:gba_time_scaling} for the multi-index information exponent $\ell$. A natural question is thus to ask whether the class of Algorithm~\ref{algo:optimizer_main_step} also allows us to bypass this requirement. We show that this is indeed the case. Consider a neural network as in Equation~\eqref{eq:def_nn}; we assume that the internal learning rate $\rho$ is chosen independently for each neuron:
\begin{assumption}
    For each $j \in [p]$, the parameter $\rho_{0, j}$ is chosen independently from all other neurons, according to a \emph{symmetric} distribution which is absolutely continuous w.r.t the Lebesgue measure.
\end{assumption}

\begin{theorem}\label{thm:multi_index_recovery}
    Let $\delta > 0$, and $\Pi^\star$ the projection operator on $V^\star$. There exists constants $\gamma_0(\delta), C(\delta)$ depending only on $\delta$ such that if we take $p \geq C(\delta)k$ and
    \begin{itemize}
        \item if $\ell_p^\star = 1$, $\gamma = \gamma_0(\delta) d^{-1}$ and $T = C(\delta)d$,
        \item if $\ell_p^\star = 2$, $\gamma = \gamma_0(\delta) (d\log(d))^{-1}$ and $T = C(\delta)d\log(d)^2$,
    \end{itemize}
    then with probability $1 - \delta$, there exists a $t \leq T$ such that at least a positive proportion of the vectors $\vec{w}_{t, i}$ satisfy $\norm{\Pi^\star \vec{w}_{t, i}} \geq \eta$.
Further, if $\ell_p^\star = 1$, then the vectors $\{\Pi^\star \vec{w}_{t, i}\}_{i \in [p]}$ span the minimal subspace $U^\star$.
\end{theorem}

\begin{figure}
    \centering
    \subfigure[ ${\scriptstyle h^\star(\vec x)= x_1 + x_1 \mathrm{He}_3(x_2)}$]{%
        \includegraphics[height=0.23\textwidth, trim={0 8 0 0}, clip]{figures/fig2_k3_kstar1_staircase.pdf}
        \label{fig:staircase_1}
    }
    \hfill \subfigure[${\scriptstyle h_{\mathrm{sign}}^\star(\vec{x}) = \mathrm{sign}(x_1x_2x_3), \quad h^\star_{\mathrm{stair}}(\vec x) = \mathrm{He}_2(x_1) + \mathrm{sign}(x_1x_2x_3)}$]{%
        \includegraphics[height=0.23\textwidth, trim={0 8 0 0}, clip]{figures/figs_SQStair_long.pdf}
        \label{fig:staircase_2}
    }
    \caption{\textbf{Hierarchical learning --} Evolution of the maximum Cosine Similarities with different target directions $\{\vec w^\star_r\}_{r \in [k]}$ are identified by different colors: $\vec w^\star_1$ (blue), $\vec w^\star_2$ (orange), $\vec w^\star_3$ (green) as a function of the normalized iteration time.
    \textbf{(a):} both the algorithms learn $\vec w^\star_1$ in linear time, but only EgD can also learn $\vec w^\star_2$ in $O(d)$ via a staircase mechanism; SGD requires another $O(d^2)$ steps to take advantage of the staircase and learn $\vec w^\star_2$.
    \textbf{(b):} EgD performance for the target function $f^\star_{\mathrm{stair}}$ (dots) and $f^\star_{\mathrm{sign}}$(squares); we plot in separate subplots the overlap with different directions to highlight the presence of hierarchical learning mechanism. Learning the first target direction $\vec w^\star_1$ triggers the hierarchical mechanism and EgD is able to weakly recover the full target subspace $\mathrm{Span}(\vec w^\star_1, \vec w^\star_2, \vec w^\star_3)$ in $O(d \log d)$, while this does not happen when removing $\mathrm{He}_2(x_1)$ from the target.
    See App.~\ref{sec:app:implementation} for additional details.}
    \label{fig:main:staircase1}
\end{figure}

\subsection{Numerical investigation with multi-index target}\label{subsec:multi_numerics}

% (\lp{Def.~\ref{def:hardness_subspace}}). 
We illustrate the results of Thm.~\ref{thm:multi_index_recovery} numerically by comparing the performance of One-Pass SGD with Alg.~\ref{algo:optimizer_main_step} in Fig~\ref{fig:main:multi_index_complete}. We measure the maximal cosine similarity between the hidden layer neurons and the different rows of the target's weight matrix $W^\star$ as a function of the iteration time. We set without loss of generality the target's directions to the standard basis of $\mathbb{R}^d$ to ease the notation. The algorithms considered are again EgD and vanilla One-Pass SGD (See App.~\ref{sec:app:implementation} for details).
\begin{itemize}[noitemsep,leftmargin=1em,wide=0pt]
\item \textbf{SGD-easy non-symmetric targets ($\ell \!=\! \ell^\star \!=\! 1$) --} Fig.~\ref{fig:main:multi_index_complete}, left, shows $h^\star(x_1,x_2) = x_1 + x_1x_2$. Here both SGD and Alg.~\ref{algo:optimizer_main_step} learn in $T= O(d)$ the directions $(\vec w^\star_1, \vec w^\star_2)$.

\item \textbf{SGD-easy symmetric targets ($\ell \!=\! \ell^\star \!=\! 2$) --} Fig.~\ref{fig:main:multi_index_complete}, center left, shows $h^\star(x_1,x_2) = x_1x_2$.  Here both SGD and Alg.~\ref{algo:optimizer_main_step} learn in $T=O(d \log d)$ the directions $(\vec w^\star_1, \vec w^\star_2)$. 

\item \textbf{Non-symmetric targets with SGD-easy and hard directions ($\ell_{\vec{v}} > 2, \ell^\star_{\vec{v}}=1$) --} Fig.~\ref{fig:main:multi_index_complete}, center-right, shows $h^\star(x_1,x_2) \!=\! x_1 \!+\! \mathrm{He}_3(x_2) $. Here both SGD and Alg.~\ref{algo:optimizer_main_step} learn in $T=O(d)$ the direction $\vec w^\star_1$, that satisfies $\ell_{\vec{w_1^\star}} = \ell_{\vec{w_1}^\star}^\star = 1$. However, since $\ell_{\vec{w_2^\star}} = 3$ while $\ell_{\vec{w_2^\star}}^\star = 1$, One-Pass SGD suffers from the limitations detailed in eq.~\eqref{eq:gba_time_scaling} and requires $\Omega(d^2)$ samples to learn the second direction $\vec w^\star_2$. This contrasts with the behaviour of Alg.~\ref{algo:optimizer_main_step} that learns also $\vec w^\star_2$ in $T=O(d)$ steps.

\item \textbf{SGD-hard symmetric targets ($\ell > 2,  \ell^\star =2$) --} The right section Fig.~\ref{fig:main:multi_index_complete} shows $h^\star(x_1,x_2,x_3) = x_1 x_2 x_3$. The Information Exponent is $\ell=3$, hence vanilla SGD does not learn any direction in the target subspace in $T=O(d \log d)$ iterations. However, Algorithms~\ref{algo:optimizer_main_step} learns in $T=O(d \log d)$ steps all the three directions $\{\vec w^\star_1, \vec w^\star_2, \vec w^\star_3\}$ since the Generative Exponents $\ell_{\vec{w}^\star_r}^\star$ are all equal to two.
\end{itemize}


\subsection{Learning hard functions through a hierarchical mechanism}\label{subsec:staircase}

The investigation of the hierarchical nature of SGD learning has attracted noticeable attention \citep{abbe2021staircase,abbe2022merged,abbe2023sgd, dandi2023twolayer}. In this paper, we portray a completely different picture in terms of computational efficiencies when data repetition is considered in the algorithmic SGD routine. One may wonder if there is a generalization of such a hierarchical learning mechanism to the present novel setting. Indeed for optimal AMP algorithm, a diffrent picture emerges, (called \emph{Grand staircase} in \cite{troiani2024fundamental}). Here we show that coupling between directions can hierarchically guide the learning process as well with SGD.

\begin{wrapfigure}{r}{0.6\textwidth} % 'r' for right, 'l' for left
    \centering
    \vspace{-.4cm}
    \includegraphics[width=\linewidth]{figures/figs_SQStairH4_long.pdf}
    \caption{\textbf{Hierarchical learning --} Evolution of the maximum Cosine Similarities attained by EgD with different target directions $\{\vec w^\star_r\}_{r \in [k]}$ are identified by different colors: $\vec w^\star_1$ (blue), $\vec w^\star_2$ (orange), $\vec w^\star_3$ (green) as a function of the normalized iteration time. The target function is $f^\star_{\mathrm{sq-stair}}(\vec z)= \mathrm{He}_4(z_1) + \mathrm{sign}(z_1z_2z_3)$, that is an SQ-staircase (or grand staircase), not a CSQ-staircase. EgD learn $\vec w^\star_1$ in \(O(d\log d)\) steps and use the information to learn the other two directions in another \(O(d\log d)\) steps. SGD (not showed in the plot) cannot take advantage of the staircase mechanism since $\mathrm{He}_4(z_1)$ and $\mathrm{sign}(z_1z_2z_3)$ have information exponent \(\ell = 4\) and \(\ell = 3\) respectively. (See App.~\ref{sec:app:implementation}).}
    \vspace{-.4cm}
    \label{fig:main:staircase2}
\end{wrapfigure}
The Left panel in Fig.~\ref{fig:main:staircase1} shows an example of the so-called staircase functions \citep{abbe2021staircase}, i.e. $f^\star(\vec z) = z_1 + z_1 \mathrm{He}_3(z_2)$. While one-pass SGD needs to learn hierarchically first the direction $\vec w^\star_1$ in $T=O(d)$ and then $\vec w^\star_2$ in $T=O(d^2)$, Algorithm~\ref{algo:optimizer_main_step} easily learns both in linear time. This observation could lead to infer that hierarchical learning mechanisms are not present when more realistic training scenarios are considered. 



To refute this, we illustrate in the right panel of Fig.~\ref{fig:main:staircase1} a scenario that precisely exemplifies the presence of hierarchical mechanisms within Algorithm~\ref{algo:optimizer_main_step}. We run this algorithm on two different target functions, $f_{\mathrm{sign}}^\star(\vec{z}) = \mathrm{sign}(z_1z_2z_3)$ and $f^\star_{\mathrm{stair}}(\vec z) = \mathrm{He}_2(z_1) + \mathrm{sign}(z_1z_2z_3)$. We show in App. \ref{sec:app:proofs} that $3-$sparse parities of the form $\mathrm{sign}(z_1z_2z_3)$ are hard functions even for SGD with data repetition (Algorithm~\ref{algo:optimizer_main_step}), and indeed they are not learned in (almost) linear time. On the other hand, for the function $f^\star_{\mathrm{stair}}$, our simulations predict that the first direction $\vec w^\star_1$ is learned in $T = O(d \log d)$ iterations (see the rightmost panel of Fig.~\ref{fig:main:multi_index_complete}). However, once the direction $\vec w^\star_1$ is learned, it can be used to obtain order-one correlation with $\{\vec w^\star_2, \vec w^\star_3\}$ again in $T = O(d \log d)$ steps. While the latter example belongs to the class of ``CSQ'' staircase function depicted in \cite{abbe2021staircase}, novel ``SQ'' hierarchical mechanisms arise in our framework, such as for instance the function $f_{\mathrm{sq-stair}}^\star(\vec z) = \mathrm{He}_4(z_1) + \mathrm{sign}(z_1z_2z_3)$ (see Fig.~\ref{fig:main:staircase2}). 

The staircase picture in terms of generative exponent was discussed for AMP-type algorithm in \cite{troiani2024fundamental}. Our study indicate that this new class (they called grand staircase) is not restricted to AMP: We anticipate that grand staircase functions can be efficiently learned by two-layer networks when data reusing is permitted, whereas only standard staircase ones emerge  under single-pass SGD. Additional recent results by \citep{joshi2024complexity}  align with this perspective. 


% \begin{figure}
%     \centering
%     \includegraphics[width=.6\textwidth]{figures/figs_SQStairH4_long.pdf}
%     \caption{\textbf{Novel hierarchical picture of learning --} Evolution of the maximum Cosine Similarities attained by EgD with different target directions $\{\vec w^\star_r\}_{r \in [k]}$ are identified by different colors: $\vec w^\star_1$ (blue), $\vec w^\star_2$ (orange), $\vec w^\star_3$ (green) as a function of the normalized iteration time. The target function is $f^\star_{\mathrm{sq-stair}}(\vec z)= \mathrm{He}_4(z_1) + \mathrm{sign}(z_1z_2z_3)$, that is an SQ-staircase, but not a CSQ-staircase. EgD learn $\vec w^\star_1$ in \(O(d\log d)\) steps and use the information to learn the other two directions in another \(O(d\log d)\) steps. SGD (not showed in the plot) cannot take advantage of the staircas mechanism since $\mathrm{He}_4(z_1)$ and $\mathrm{sign}(z_1z_2z_3)$ have information exponent \(\ell = 4\) and \(\ell = 3\) respectively. See App.~\ref{sec:app:implementation} for additional details.}
%     \label{fig:main:staircase2}
    
% \end{figure}



==> sections_old/sections/setting.tex <==
\section{Setting and Main Contributions}
\label{sec:main:setting}

Given a dataset of $N$ labeled examples $\{\vec z^\nu, y^\nu\}_{\nu \in [N]}$ in $d$ dimensions, we analyze the learning properties of fully connected two-layer networks with first layer weights $W=\{\vec w_j\}_{j \in [p]}$, second layer $\vec a \in \mathbb{R}^p$, and activation function $\sigma: \mathbb R \to \mathbb R$
\begin{align}
    f(\vec z; W, \vec a) = \frac{1}{p} \sum_{j =1}^p a_j \sigma \left(\langle \vec z, \vec w_j \rangle \right) \label{eq:def_nn}
\end{align}
We consider target functions that are dependent only on few orthogonal relevant directions $k=O_d(1)$ encoded in the target's weight matrix $W^\star = \{\vec w^\star_r\}_{r \in [k]} \in \mathbb{R}^{k\times d}$:
\begin{align}
    y^\nu = f^\star(\vec z^\nu) = h^\star(W^\star \vec z^\nu)
\end{align}
This model for structured data is usually referred to as a \textit{multi-index} model. Our main objective will be to analyze how efficiently two-layer nets adapt to this low-dimensional structure during training. To ensure that all necessary Gaussian expectations exist, we make the following non-restrictive assumption on $\sigma, h^\star$:
\begin{assumption}\label{assump:poly_growth}
    The functions $\sigma$ and $h^\star$ have at most polynomial growth, in the sense that there exists a constant $C > 0$ such that for all $x \in \mathbb{R}, \vec{x} \in \mathbb{R}^k$,
    \begin{equation}\label{eq:poly_growth}
        |\sigma(x)| \leq C(1 + |x|)^C \quad \text{and} \quad |h^\star(\vec{x})| \leq C(1 + \|\vec{x}\|)^C.
    \end{equation} 
\end{assumption}
\paragraph{Training algorithm --}
Our goal is to minimize the following objective:
\begin{equation}
    \cR(W, \vec{a}) = \E_{\vec{z}, y}\left[ \cL(f(\vec{z}, W, \vec{a}), y) \right]
\end{equation}
where $\cL: \R \times \R \to \R$ is a loss function, and the expectation is over the data distribution.

This objective is non-convex, and we do not have direct access to the expectation over the data. A central question in Machine Learning is therefore to quantify the properties of the weights attained at convergence by different algorithms. In this manuscript we consider a specific class of one-pass training routines to minimize the empirical risk. First, we partition the dataset in disjoint mini-batches of size $n_b$, i.e. $\mathcal{D} = \cup_{t \in [T]}\{\vec x^\nu, y^\nu\}_{\nu \in [tn_b, (t+1)n_b]}$ where $T$ is the total number of iterations considered. For each algorithmic step, we update the hidden layer neurons $W=\{\vec w_j\}_{j \in [p]}$ with the program $\mathcal{A}: (\vec w_{j,t}, \gamma, \rho, n_b) \in \mathbb{R}^{d+3} \to \vec w_{t+1,j} \in \mathbb{R}^d$.
\begin{myalgorithm}[Optimizer Main Step]
\label{algo:optimizer_main_step}
 \begin{equation}
 \begin{aligned}
     \vec w_{t+1,j} & =  \mathcal{A}(\vec w_t, \gamma, \rho, n_b) 
     =  \vec w_{t,j} - \frac{\gamma }{n_b}\sum_{\nu \in [n_b]
     }\nabla_{\vec w_{t,j}}
     \cL
    \left(
    f (\vec z^\nu; 
    \Tilde{W}_t(\rho), \vec a_0 ),  y^\nu  \right) \\
   \Tilde{\vec{w}}_{t, j} (\rho) &= \vec{w}_{t, j} - \rho \nabla_{\vec w_{t,j}}
    \cL\left( f(\vec z^\nu; W_t, \vec a_0),  y^\nu \right)
 \end{aligned}
\label{eq:algorithm}     
 \end{equation}
\end{myalgorithm}
This class of algorithms defined by the optimizer step $\mathcal{A}(\cdot\,, \gamma, \rho, n_b)$, in which we consider the final gradient update after taking a linear combination of the current iterate and its current gradient (noted as $\Tilde{W}_t(\rho)$ in the above), is broadly used in different contexts. Indeed, routines with positive $\rho$ parameters correspond to Extragradient methods (EgD) \citep{Korpelevich1976TheEM}, while with negative $\rho$ have been recently used in the context of Sharpness Aware Minimization (SAM) \citep{foret2021sharpnessaware}. For clarity, we present our theoretical results with the above, easily interpretable, Algorithm~\ref{algo:optimizer_main_step}. However, our theoretical claims are valid in a more general setting; we refer to Appendices~(\ref{sec:app:proofs}, \ref{sec:app:numerics}) for additional results on more general optimizer steps. 
% The complete description of the algorithmic routine is given in App.~\ref{sec:app:numerics} (See Algorithm~\ref{algo:full_algorithm}).

As previously stated, the central object of our analysis is the efficiency of the network to adapt to the low-dimensional structure identified by $W^\star$. Therefore, we focus on the learned representations by the first layer weights $W_t$ while keeping the second layer weights $\vec a_t = \vec a_0$ fixed during training. This assumption is favorable to performing the theoretical analysis and is largely used in the theoretical community (e.g., \cite{damian2022neural, ba2022high, Bietti2022}).

Numerous theoretical efforts have been devoted to understanding the sample complexity needed to learn multi-index targets. However, an important aspect of many algorithmic routines considered is to exploit a clever \textit{warm start} to initialize the iterates \citep{mondelli2018fundamental, luo2019optimal, maillard2020phase, chen2020learning}. We show in this work that such preprocessing of the data is not needed to learn all polynomial multi-index functions in $T=O(d \log d)$ with the routine in Alg.~\ref{algo:optimizer_main_step}. Instead, we consider a fully agnostic initialization of the network:

\begin{assumption}\label{assump:init}
For each $j \in [p]$, the initial first-layer weight $\vec{w}_{0, j}$ is initialized according to the uniform measure on the sphere:
\[ \vec{w}_{0, j} \overset{i.i.d}{\sim}\operatorname{Unif}(\mathbb{S}^{d-1}). \]
The second-layer weights are drawn i.i.d in $\{-1, 1\}$:
\[ a_{0, j} \overset{i.i.d}{\sim}\operatorname{Unif}(\{-1, 1\}). \]
\end{assumption}

\paragraph{Weak recovery in high dimensions --}
The essential object in our analysis is the evolution of the correlation between the hidden neurons $W = \{\vec w_j\}_{j \in [p]}$ and the target's weights $W^\star$, as a function of the algorithmic time steps. More precisely, we are interested in the number of algorithmic steps needed to achieve an order one correlation with the target's weights $W^\star$, known as \textit{weak recovery}. 
\begin{definition}[Weak recovery]
\label{def:weak_recovery}
    The \textit{target subspace} $V^\star$ is defined as the span of the rows of the target weights $W^\star$:
    \begin{align}
    \label{eq:main:teacher_subspace_def}
        V^\star = \operatorname{span}(\vec w^\star_1, \dots, \vec w^\star_k)
    \end{align}
    We define the weak recovery stopping time for a parameter $\eta \in (0,1)$ independent from $d$ as:
\begin{equation}
    t^{+}_{\eta} = \operatorname{min}\{t \geq 0: \lVert W W^{\star \top} \lVert_F \geq \eta\}
\end{equation}
\end{definition}

\paragraph{From Information Exponents to Generative Exponents --}Recent works have sharply theoretically characterized the weak recovery stopping time for a variety of multi-index targets learned with one-pass SGD. \cite{BenArous2021} for the single-index case, then \cite{abbe2022merged} for the multi-index one have unveiled the presence of an Information Exponent $\ell$ characterizing the time complexity needed to weakly recover the target subspace $V^\star$, defined in the single-index case as
\begin{equation}
    \ell = \min \{ k \in \N \::\: \Eb{x \sim \cN(0, 1)}{h^\star(x)H_k(x)} \neq 0 \}.
\end{equation}
where $H_k$ is the $k$-th Hermite polynomial \citep{odonnell_2014_analysis}.
Under this framework, the sample complexity required to achieve weak recovery when the link function has Information Exponent $\ell$ is \citep{BenArous2021}
\begin{align} \label{eq:gba_time_scaling}
    T(\ell) = 
        \begin{cases}
        &O(d^{\ell -1} ) \qquad \hspace{0.8em}\text{if $\ell>2$} \\
        &O(d \log{d} ) \qquad \text{if $\ell=2$} \\
        &O(d) \qquad \hspace{2.2em}\text{if $\ell=1$}.
    \end{cases}
\end{align}
These bounds have been improved by \cite{damian_2023_smoothing} up to order $d^{\ell/2}$; the latter matches the so-called \emph{Correlated Statistical Query} lower bound, which considers queries of the form $\Ea{y \phi(\vec{z})}$.

However, this Information Exponent is not the right measure of complexity for low-dimensional weak recovery. Some iterative algorithms, for instance, are known to perform drastically better\citep{barbier2019optimal,celentano2021highdimensional,mondelli2018fundamental,luo2019optimal,maillard2020phase,troiani2024fundamental}. Recently \cite{damian2024computational} introduced a new Generative Exponent $\ell^\star$ (generative exponent) governing the weak recovery time scaling for algorithms in the Statistical Query (SQ) or Low Degree Polynomial (LDP) family. This exponent is defined as
\begin{equation}
    \ell^\star = \min \{ k \in \N \::\: \Eb{x \sim \cN(0, 1)}{f(h^\star(x))H_k(x)} \neq 0 \ \text{for some} \ f: \R \to \R \},
\end{equation}
which allows for the application of arbitrary transformations of the labels before performing the queries. Under this definition, the ``hard'' problems with $\ell^\star > 2$ are also impossible to learn for the best first-order algorithm, \emph{Approximate Message Passing} \citep{troiani2024fundamental}. 

We discuss in this work the extension of the generative exponent to the multi-index setting and investigate the dynamics of specific gradient-based programs (Algorithm~\ref{algo:optimizer_main_step}) as a function of the freshly defined hardness exponent $\ell^*$. 
These theoretical findings match the recent one of \cite{kou2024matching} on the computational efficiency of SGD in learning sparse $k-$parity (associated with $\ell^\star = k$).

When the optimal transformation $f$ is known, a simple SGD algorithm on $(\vec{z}, f(y))$ achieves the Generative Exponent lower bound. However, one problem remains: does there exist a class of SGD-like algorithms that can achieve this lower bound agnostically?

\paragraph{Achieving lower bounds with data repetition --}

Although the performance of single-pass SGD is limited by the Information Exponent of $h^\star$, the situation drastically changes when multiple-pass algorithms are considered. Recently, \cite{dandi2024benefits} proved that non-even single-index targets are weakly recovered in $T = O(d)$ when considering extensive batch sizes with multiple pass. This begs the question of how good can a ``reusing'' algorithm be. We answer this question for the class of polynomial link functions:
\begin{theorem}[Informal]
    There is a choice of hyperparameters such that if $h^\star$ is a polynomial function, Algorithm~\ref{algo:optimizer_main_step} achieves weak recovery in $O(d\log(d)^2)$ samples.
\end{theorem}
This shows in particular that a simple gradient-based algorithm, which only requires seeing the data twice, is optimal for learning any polynomials.

\paragraph{Learning representations --}
Learning relevant features from data is a fundamental property of neural networks. However, much theoretical work has focused on lazy training in two-layer networks \citep{jacot2018neural}, where features are not effectively learned. In this regime, shallow networks behave as kernel machines, which struggle to adapt to low-dimensional structures in data \citep{Ghorbani2020}. Understanding representation learning and corrections to the kernel regime is thus a key challenge in machine learning theory \citep{pmlr-v75-dudeja18a, atanasov2022neural, Bietti2022, damian2022neural, petrini2022learning}. In this manuscript we provably characterize the number of iterations needed from Algorithm~\ref{algo:optimizer_main_step} to learn the relevant features of the data, i.e., attain weak recovery of the target subspace. Our results provide the scaling of the relevant hyperparameters $(\gamma, \rho)$ with the diverging input dimension $d$. The minibatch size will be fixed to $n_b =1$ in the main body, and we refer to Appendix~\ref{sec:app:numerics} for the extension to larger batch sizes.


\subsection*{Summary of Main Results}
\begin{itemize}[noitemsep,leftmargin=1em,wide=0pt]
    \item We prove for single-index targets that one-pass gradient-based algorithms surpass the Correlation Statistical Query (CSQ) limits established by the Information Exponent \citep{BenArous2021}.  
    \item We unveil that the dynamics of the family of Alg.~\ref{algo:optimizer_main_step} are governed by the generative exponent \cite{damian2024computational}, with an additional polynomial restriction on the transformation of the output.
    \item We generalize the notion of generative exponent to multi-index targets. As in the single-index case, one-pass gradient-based algorithms can overcome CSQ performance dictated by the Leap Coefficient \citep{abbe2022merged}. Our definition is consistent with the one of \citep{troiani2024fundamental}. 
    \item We prove that all polynomial multi-index functions are learned by Algorithm~\ref{algo:optimizer_main_step} either with total sample complexity $O(d)$ or $O(d \log(d)^2)$ if associated with the presence of a symmetry. 
    \item  The implementation of Algorithm~\ref{algo:optimizer_main_step} does not require pre-processing to initially correlate the estimation with the ground truth, and learns the meaningful representations from data alone. This is in contrast numerous findings (e.g., \cite{mondelli2018fundamental, luo2019optimal, maillard2020phase} for single index targets or \cite{chen2020learning} for multi-index ones).
    \item We characterize the class of hard functions not learned  in (almost) linear sample complexity. We show, however, that such functions can be learned through an hierarchical mechanism that extends the CSQ staircase first developed in \cite{abbe2021staircase} to a different, larger set, of functions.
    \item We validate the formal theoretical claims with detailed numerical illustrations. The code to reproduce representative figures is available at \href{https://anonymous.4open.science/r/repetita-iuvant}{https://anonymous.4open.science/r/repetita-iuvant}.
\end{itemize}

==> sections_old/sections/single_index.tex <==
\section{Single-Index Model}
\subsection{Main results}
We first consider, for simplicity, the class of single-index models, in which $k \!=\! p \!=\! 1$. This corresponds to a mismatched setting of Generalized Linear Models, in which we want to learn
\[ y = h^\star(\langle \vec{w^\star}, \vec{z} \rangle), \quad \text{with} \quad f(\vec{z}, \vec{w}, a) = a\sigma(\langle \vec{w}, \vec{z} \rangle). \]
In this section we rigorously characterize the number of iterations needed for the class of Algorithms~\ref{algo:optimizer_main_step} to perform weak recovery (as in Definition~\ref{def:weak_recovery}) in the context of single-index targets. We establish a clear separation between the the learning efficiency of the algorithmic  family~\ref{algo:optimizer_main_step} and One-Pass SGD, limited by the Information Exponent of the target to be learned \citep{BenArous2021}.

We start by introducing a restriction of the generative information exponent in \cite{damian2024computational} to polynomial transformations.
\begin{definition}[Polynomial Generative Information exponent]
\label{def:lstar_damian2024}
We define $\ell^\star_p$ as the smallest integer $k$ such that there exists a polynomial $p: \R \rightarrow \R$ with:
\begin{equation}\label{eq:f_hard_gen}
        \Eb{x\sim\cN(0, 1)}{p(h^\star(x))H_{k}(x)}\neq 0,
    \end{equation}
\end{definition}

Our assumptions on the SGD implementation and the target function are as follows:
\begin{assumption}\label{assump:spherical_corr}
    Algorithm \ref{algo:optimizer_main_step} is run with single-sample steps ($n_b = 1$), and uses the correlation loss
    \[ \cL(y, \hat y) = 1 - y\hat y.\]
    We also consider a spherical version of Alg. \ref{algo:optimizer_main_step}, with
    \begin{equation}\label{eq:spherical_sam}
        \vec{w}_{t+1} = \frac{\vec w_{t} - \gamma\nabla^\bot_{\vec w}
     \cL
    \left(
    f (\vec z^\nu; 
    \tilde{\vec{w}}_t(\rho), a_0),  y^\nu  \right)}{\norm{\vec w_{t} - \gamma\nabla^\bot_{\vec w}
     \cL
    \left(
    f (\vec z^\nu; 
    \tilde{\vec{w}}_t(\rho), a_0),  y^\nu  \right)}}
    \end{equation}
    where $\nabla^\bot f = \nabla f - \langle \nabla f, \vec{w} \rangle \vec{w}$ is the spherical gradient.
\end{assumption}

\begin{assumption}\label{assump:derivatives}
    The activation $\sigma$ is analytic almost everywhere, and $\sigma^{(n)}$ satisfies the polynomial growth assumption \eqref{eq:poly_growth} for $n \in \mathbb{N}$ (possibly for different constants $C_n$). Further, for all $n \geq 1$, we have
    \[ \Eb{x\sim\cN(0, 1)}{\sigma^{(n)}(x) \sigma'(x)^{n-1}} \neq 0 \quad \text{and} \quad \Eb{x\sim\cN(0, 1)}{x \sigma^{(n)}(x) \sigma'(x)^{n-1}} \neq 0 \]
\end{assumption}

We are now ready to state our main result.
\begin{theorem}
\label{thm:single_index_recovery}
    Suppose that Assumptions \ref{assump:poly_growth}-\ref{assump:derivatives} hold, and let $\rho = \rho_0 d^{-1}$. Then, under an event of probability $1/2$ on the initialization $(a_0, \vec{w}_0)$, for each $\delta > 0$, there exist constants $\gamma_0(\delta)$ and $C(\delta)$ such that the following holds:
    \begin{itemize}
        \item If $\ell_p^\star = 1$, choosing $\gamma = \gamma_0(\delta)d^{-1}$, then
$
             \dP(t^+_\eta \leq C(\delta) \cdot d) \geq 1 - \delta
     $,

        \item If $\ell_p^\star = 2$, choosing $\gamma = \gamma_0(\delta)[d\log(d)]^{-1}$, then 
        $
            \dP(t^+_\eta \leq C(\delta) \cdot d \log(d)^2) \geq 1 - \delta
       $.
    \end{itemize}
    The above holds for almost every choice of $\rho_0$ under the Lebesgue measure. In particular, in a network with $p = O(\log\frac1\delta)$ neurons, at least one of them achieves weak recovery with probability $1 - \delta$.
\end{theorem}

\paragraph {Proof Sketch --} We provide here the proof sketch for Theorem~\ref{thm:single_index_recovery}. For any vector $\vec{w}$, under the correlation loss, we have
\begin{equation}\label{eq:sgd_gradient}
    \nabla_{\vec{w}} \cL(f(\vec{z}; \vec{w}, a_0), y) = a_0 y \sigma'(\langle \vec{w}, z \rangle) \cdot \vec{z},
\end{equation}
so the gradient is aligned with $\vec{z}$. As a result, we have
\begin{equation}\label{eq:sam_gradient}
    \nabla_{\vec w}\cL\left(f(\vec z; \tilde{\vec{w}}(\rho), a_0),  y \right) = a_0 y \sigma'\big(\langle \vec{w}, \vec{z} \rangle + a_0 \rho y \sigma'(\langle \vec{w}, \vec{z} \rangle) \cdot \underbrace{\norm{\vec{z}}^2}_{\approx d}\big) \cdot \vec{z}
\end{equation}
This expression for the gradient exhibits two important properties:
\begin{itemize}
    \item Even though $\rho \asymp d^{-1}$, since the gradient lies along $\vec{z}$, the additional dot product with $\vec{z}$ amplifies the signal by a factor of $d$,
    \item The resulting gradient  \eqref{eq:sam_gradient} is a \emph{non-linear} function of $y$, as opposed to the linear one of \eqref{eq:sgd_gradient}. 
\end{itemize}
The latter property enables us to show that the dynamics driven by equation \eqref{eq:sam_gradient} can implement all polynomial transformations of the output $y$, for almost all choices of $\rho_0$. Subsequently, the SGD algorithm on the transformed input $p(y)$ can be studied with the same techniques as \cite{BenArous2021}, but with an information exponent equal to $\ell_p^\star$.

\subsection{Discussion}\label{subsec:single_index_discussion}

\paragraph{Significance and necessity of the assumptions --}
Assumption \ref{assump:spherical_corr} simplifies Alg.~\ref{algo:optimizer_main_step} to a more tractable version. In particular, the normalization step allows us to keep track of only one parameter, the overlap between $\vec{w}_t$ and $\vec{w}^\star$. We expect however Thm.~\ref{thm:single_index_recovery} to hold in the general setting of Alg.~\ref{algo:optimizer_main_step}.

Assumption \ref{assump:derivatives} is a regularity assumption, ensuring that some quantities of interest in the proof are non-zero. The first part is satisfied by virtually every activation function; the second is more restrictive, but we show that it is satisfied for biased activations:
\begin{lemma}\label{lem:bias_activation}
    Let $\sigma$ be a non-polynomial analytic function. Then the second part of Assumption \ref{assump:derivatives} is true for the function $x \mapsto \sigma(x + b)$ for almost every choice of $b$ (according to the Lebesgue measure).
\end{lemma}

Finally, although we state our result as an almost sure event over $\rho_0$, it can be reformulated into an event on the second layer weight $a_0$, in which the randomness comes from the initialization step.

\paragraph {Learning polynomial functions --} Although our definition of the Polynomial Generative Information exponent is more restrictive than the one in \cite{damian2024computational}, we show that it is enough to allow learning of a large class of functions, namely polynomials:
\begin{theorem}\label{thm:poly_pge}
    Assume that $h^\star$ is a polynomial function. Then the Polynomial Generative Information exponent of $h^\star$ is always at most 2, and is equal to 1 whenever $h^\star$ is not even.
\end{theorem}
This theorem implies that the Extragradient algorithm class allows us to match the sample complexity of the algorithm of \cite{chen2020learning}, without the need for \emph{ad hoc} preprocessing.

\paragraph{Comparison with \cite{lee2024neural}} \cite{lee2024neural} independently obtained results on the \emph{strong} recovery for single index models. However, this  requires either perfect knowledge of the link function $h^\star$ or a very ad-hoc neural network, in which each neuron has a different polynomial activation of large degree with random coefficients. In contrast, apart from a $1/2$ probability event on the initialization, all our results hold with probability one on the choice of initial biases or parameter $\rho$.

\paragraph{Beyond Algorithm~\ref{algo:optimizer_main_step} --} A succinct summary of the proof goes as follows: the first time we see a sample $\vec{z}$, we store information about $y$ along the direction of $\vec{z}$. The second time we see the same sample, the component along $\vec{z}$ in $\vec{w}$ interact \emph{non-linearly} with $y$, which bypasses the CSQ framework. Importantly, we expect that this behavior also appears in SGD algorithms where we do not see the data twice \emph{in a row}, but \emph{across multiple epochs}! Indeed, upon small enough correlation between the $\vec{z}^\nu$, seeing multiple examples before the repetition of $\vec{z}$ should not interfere with the data stored along this direction.
We are therefore not claiming that Algorithm~\ref{algo:optimizer_main_step} is superior to other classically-used methods; rather, it provides a tractable and realistic setting to study data repetition in SGD, which was ignored in previous theoretical works on the topic. 

\begin{figure}[t]
    \centering
    \subfigure[$\scriptstyle h^\star(x) = \operatorname{relu}(x)$]{%
        \includegraphics[height=0.21\textwidth]{figures/fig1_ReluRelu.pdf}
        \label{fig:single_index_1}
    }\hfill
    \subfigure[$\scriptstyle h^\star(x) = \mathrm{He}_2(x)$]{%
        \includegraphics[height=0.21\textwidth]{figures/fig1_H2Relu.pdf}
        \label{fig:single_index_2}
    }\hfill
    \subfigure[$\scriptstyle h^\star(x) = \mathrm{He}_3(x)$]{%
        \includegraphics[height=0.21\textwidth]{figures/fig1_H3Relu.pdf}
        \label{fig:single_index_3}
    }\hfill
    \subfigure[$\scriptstyle h^\star(x) = \mathrm{He}_4(x)$]{%
        \includegraphics[height=0.21\textwidth]{figures/fig1_H4Relu.pdf}
        \label{fig:single_index_4}
    }

    \caption{\textbf{Learning single-index targets --}
    Evolution of the Cosine Similarity attained by EgD (crosses) and SGD (dots) as a function of the normalized iteration time.
    (dashed horizontal line $\frac{1}{\sqrt{d}}$ is a visual guide to place random performance).
    \textbf{(a) $(\ell,\ell^\star)=(1,1)$:} both algorithms learn in linear time.
    \textbf{(b) $(\ell,\ell^\star)=(2,2)$:} both algorithms learn in $O(d\log d)$ time.
    \textbf{(c) $(\ell,\ell^\star)=(3,1)$:} EgD learns in linear time, while SGD requires $O(d^2)$ time.
    \textbf{(d) $(\ell,\ell^\star)=(4,2)$:} EgD learns in $O(d\log d)$ time,  SGD requires $O(d^3)$ time
    (Details in App.~\ref{sec:app:implementation}).}
    \label{fig:main:single_index_complete}
\end{figure}



% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.21\textwidth}
%     \includegraphics[height=0.95\textwidth]{figures/fig1_ReluRelu.pdf}
%         \caption{$h^\star(x) = \operatorname{relu}(x)$}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.21\textwidth}
%         \includegraphics[height=0.95\textwidth]{figures/fig1_H2Relu.pdf}
%         \caption{$h^\star(x) = \mathrm{He}_2(x)$}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.21\textwidth}
%     \includegraphics[height=0.95\textwidth]{figures/fig1_H3Relu.pdf}
%         \caption{$h^\star(x) = \mathrm{He}_3(x)$}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.21\textwidth}
%         \includegraphics[height=0.95\textwidth]{figures/fig1_H4Relu.pdf}
%         \caption{$h^\star(x) = \mathrm{He}_4(x)$}
%     \end{subfigure}
%     \caption{\textbf{Learning single-index targets --}
%     Evolution of the Cosine Similarity attained by EgD (crosses) and SGD (dots) as a function of normalized iteration time.
%     The dashed horizontal line $\frac{1}{\sqrt{d}}$ is a visual guide to place random performance.
%     \textbf{(a) $(\ell,\ell^\star)=(1,1)$:} both the algorithm learn in linear time.
%     \textbf{(b) $(\ell,\ell^\star)=(2,2)$:} both the algorithm learn in \(O(d\log d)\) time.
%     \textbf{(c) $(\ell,\ell^\star)=(3,1)$:} EgD learns in linear time, while SGD would learn the same function in quadratic time.
%     \textbf{(d) $(\ell,\ell^\star)=(4,2)$:} EgD learns in \(O(d\log d)\) time, while SGD would learn in \(O(d^3)\) time.
%     See all the details in App.~\ref{sec:app:implementation}.}
%     \label{fig:main:single_index_complete}
% \end{figure}

\subsection{Numerical illustrations}\label{subsec:single_numerics}
We illustrate in Fig.~\ref{fig:main:single_index_complete} the stark difference between the weak recovery dynamics of One-Pass SGD and Algo.~\ref{algo:optimizer_main_step} for single-index targets. The Cosine Similarity between the learned weight $\vec w_t$ and the ground truth informative direction $\vec w_\star$ is shown as a function of the time steps $t$ for different target functions. Two optimization routines are considered to exemplify the learning behaviour: a) Extragradient Descent (EgD), corresponding to the family of Algorithms~\ref{algo:optimizer_main_step} with positive $\rho$ parameters; b) One-Pass SGD, corresponding to vanilla SGD, or equivalently Algorithm~\ref{algo:optimizer_main_step} associated with $\rho=0$ hyperparameter. The scaling of $(\gamma, \rho)$ as a function of the input dimension  $d$ and exponent $\ell^\star$ are given in Thm.~\ref{thm:single_index_recovery}, while the mini-batch size is fixed to $n_b =1$ (See App.~\ref{sec:app:numerics} for extension to larger $n_b$). For all plots, we take $\sigma=\mathrm{relu}$ and we refer to App.~\ref{sec:app:implementation} for details.
\begin{itemize}[noitemsep,leftmargin=1em,wide=0pt]
    \item \textbf{SGD-easy non-symmetric targets ($\ell = \ell^\star =1$) --} The Left section of Fig.~\ref{fig:main:single_index_complete} shows $h^\star(x) = \mathrm{relu}(x)$. Here both SGD and Algorithm~\ref{algo:optimizer_main_step} learn in $T= O(d)$.
    \item \textbf{SGD-easy symmetric targets ($\ell = \ell^\star = 2$) -- } The Center-Left section of Fig.~\ref{fig:main:single_index_complete} shows $ h^\star(x) = \mathrm{He}_2(x)$. Here both SGD and Algorithm~\ref{algo:optimizer_main_step} learn in $T=O(d \log d)$. 
    \item \textbf{SGD-hard non-symmetric targets ($\ell > 2, \ell^\star =1$) -- }  The Center-Right section of Fig.~\ref{fig:main:single_index_complete} shows $ h^\star(x) = \mathrm{He}_3(x)$. Here Algortihm~\ref{algo:optimizer_main_step} learns in $T=O(d)$ while One Pass SGD suffers from the limitations detailed in eq.~\eqref{eq:gba_time_scaling}, i.e. $T= O(d^{\ell-1})$ with $\ell=3$ for this case.
    \item \textbf{SGD-hard symmetric targets ($\ell > 2, \ell^\star =2$) -- } The Right section of Fig.~\ref{fig:main:single_index_complete} shows $h^\star(x) = \mathrm{He}_4(x)$. Here Algortihm~\ref{algo:optimizer_main_step} learns in $T=O(d \log d)$ while One Pass SGD suffers from the time scaling law detailed in eq.~\eqref{eq:gba_time_scaling} $T= O(d^{\ell-1})$.
\end{itemize}

    






==> sections_old/setting.tex <==
\section{Setting and Main Contributions}
\label{sec:main:setting}

Given a dataset of $N$ labeled examples $\{\vec z^\nu, y^\nu\}_{\nu \in [N]}$ in $d$ dimensions, we analyze the learning properties of fully connected two-layer networks with first layer weights $W=\{\vec w_j\}_{j \in [p]}$, second layer $\vec a \in \mathbb{R}^p$, and activation function $\sigma: \mathbb R \to \mathbb R$
\begin{align}
    f(\vec z; W, \vec a) = \frac{1}{p} \sum_{j =1}^p a_j \sigma \left(\langle \vec z, \vec w_j \rangle \right) \label{eq:def_nn}
\end{align}
We consider target functions that are dependent only on few orthogonal relevant directions $k=O_d(1)$ encoded in the target's weight matrix $W^\star = \{\vec w^\star_r\}_{r \in [k]} \in \mathbb{R}^{k\times d}$:
\begin{align}
    y^\nu = f^\star(\vec z^\nu) = h^\star(W^\star \vec z^\nu)
\end{align}
This model for structured data is usually referred to as a \textit{multi-index} model. Our main objective will be to analyze how efficiently two-layer nets adapt to this low-dimensional structure during training. To ensure that all necessary Gaussian expectations exist, we make the following non-restrictive assumption on $\sigma, h^\star$:
\begin{assumption}\label{assump:poly_growth}
    The functions $\sigma$ and $h^\star$ have at most polynomial growth, in the sense that there exists a constant $C > 0$ such that for all $x \in \mathbb{R}, \vec{x} \in \mathbb{R}^k$,
    \begin{equation}\label{eq:poly_growth}
        |\sigma(x)| \leq C(1 + |x|)^C \quad \text{and} \quad |h^\star(\vec{x})| \leq C(1 + \|\vec{x}\|)^C.
    \end{equation} 
\end{assumption}
\paragraph{Training algorithm --}
Our goal is to minimize the following objective:
\begin{equation}
    \cR(W, \vec{a}) = \E_{\vec{z}, y}\left[ \cL(f(\vec{z}, W, \vec{a}), y) \right]
\end{equation}
where $\cL: \R \times \R \to \R$ is a loss function, and the expectation is over the data distribution.

This objective is non-convex, and we do not have direct access to the expectation over the data. A central question in Machine Learning is therefore to quantify the properties of the weights attained at convergence by different algorithms. In this manuscript we consider a specific class of one-pass training routines to minimize the empirical risk. First, we partition the dataset in disjoint mini-batches of size $n_b$, i.e. $\mathcal{D} = \cup_{t \in [T]}\{\vec x^\nu, y^\nu\}_{\nu \in [tn_b, (t+1)n_b]}$ where $T$ is the total number of iterations considered. For each algorithmic step, we update the hidden layer neurons $W=\{\vec w_j\}_{j \in [p]}$ with the program $\mathcal{A}: (\vec w_{j,t}, \gamma, \rho, n_b) \in \mathbb{R}^{d+3} \to \vec w_{t+1,j} \in \mathbb{R}^d$.
\begin{algorithm}[Optimizer Main Step \textcolor{purple}{Move to appendices $n_b >1$}]
\label{algo:optimizer_main_step}
 \begin{equation}
 \begin{aligned}
     \vec w_{t+1,j} & =  \mathcal{A}(\vec w_t, \gamma, \rho, n_b) \\
     &=  \vec w_{t,j} - \frac{\gamma }{n_b}\sum_{\nu \in [n_b]
     }\nabla_{\vec w_{t,j}}
     \cL
    \left(
    f (\vec z^\nu; 
    \Tilde{W}_t(\rho), \vec a_0 ),  y^\nu  \right) \\
   \Tilde{\vec{w}}_{t, j} (\rho) &= \vec{w}_{t, j} - \rho \nabla_{\vec w_{t,j}}
    \cL\left( f(\vec z^\nu; W_t, \vec a_0),  y^\nu \right)
 \end{aligned}
\label{eq:algorithm}     
 \end{equation}
\end{algorithm}
This class of algorithms defined by the optimizer step $\mathcal{A}(\cdot\,, \gamma, \rho, n_b)$, in which we consider the final gradient update after taking a linear combination of the current iterate and its current gradient (noted as $\Tilde{W}_t(\rho)$ in the above), is broadly used in different contexts. Indeed, routines with positive $\rho$ parameters correspond to Extragradient methods (EgD) \citep{Korpelevich1976TheEM}, while with negative $\rho$ have been recently used in the context of Sharpness Aware Minimization (SAM) \citep{foret2021sharpnessaware}. For clarity, we present our theoretical results with the above, easily interpretable, Algorithm~\ref{algo:optimizer_main_step}. However, our theoretical claims are valid in a more general setting; we refer to Appendices~(\ref{sec:app:proofs}, \ref{sec:app:numerics}) for additional results on more general optimizer steps. 
% The complete description of the algorithmic routine is given in App.~\ref{sec:app:numerics} (See Algorithm~\ref{algo:full_algorithm}).

As previously stated, the central object of our analysis is the efficiency of the network to adapt to the low-dimensional structure identified by $W^\star$. Therefore, we focus on the learned representations by the first layer weights $W_t$ while keeping the second layer weights $\vec a_t = \vec a_0$ fixed during training. This assumption is favorable to performing the theoretical analysis and is largely used in the theoretical community (e.g., \cite{damian2022neural, ba2022high, Bietti2022}).

Numerous theoretical efforts have been devoted to understanding the sample complexity needed to learn multi-index targets. However, an important aspect of many algorithmic routines considered is to exploit a clever \textit{warm start} to initialize the iterates \citep{mondelli2018fundamental, luo2019optimal, maillard2020phase, chen2020learning}. We show in this work that such preprocessing of the data is not needed to learn all polynomial multi-index functions in $T=O(d \log d)$ with the routine in Alg.~\ref{algo:optimizer_main_step}. As a way to show this, we consider the extreme case in which the initial iterates $W_0$ lives in the orthogonal subspace of the target's weights $W^\star$, i.e., the `coldest' possible start.

\paragraph{Weak recovery in high dimensions --}
The essential object in our analysis is the evolution of the correlation between the hidden neurons $W = \{\vec w_j\}_{j \in [p]}$ and the target's weights $W^\star$, as a function of the algorithmic time steps. More precisely, we are interested in the number of algorithmic steps needed to achieve an order one correlation with the target's weights $W^\star$, known as \textit{weak recovery}. 
\begin{definition}[Weak recovery]
\label{def:weak_recovery}
    The \textit{target subspace} $V^\star$ is defined as the span of the rows of the target weights $W^\star$:
    \begin{align}
    \label{eq:main:teacher_subspace_def}
        V^\star = {\rm span}(\vec w^\star_1, \dots, \vec w^\star_k)
    \end{align}
    We define the following weak recovery stopping time for a parameter $\eta \in (0,1)$ independent from $d$:
\begin{equation}
    t^{+}_{\eta} = \operatorname{min}\{t \geq 0: \lVert W W^{\star \top} \lVert_F \geq \eta\}
\end{equation}
\end{definition}

\paragraph{From Information Exponents to Generative Exponents --}Recent works have sharply theoretically characterized the weak recovery stopping time for a variety of multi-index targets learned with one-pass Stochastic Gradient Descent. First \cite{BenArous2021} for the single-index case, then \cite{abbe2022merged} for the multi-index one have unveiled the presence of an Information Exponent $\ell$ characterizing the time complexity needed to weakly recover the target subspace $V^\star$, defined in the single-index case as
\begin{equation}
    \ell = \min \{ k \in \N \::\: \Eb{x \sim \cN(0, 1)}{h^\star(x)H_k(x)} \neq 0 \}.
\end{equation}
where $H_k$ is the $k$-th Hermite polynomial \citep{odonnell_2014_analysis}.
Under this framework, the sample complexity required to achieve weak recovery when the link function has Information Exponent $\ell$ is \citep{BenArous2021}
\begin{align} \label{eq:gba_time_scaling}
    T(\ell) = 
        \begin{cases}
        &O(d^{\ell -1} ) \qquad \hspace{0.8em}\text{if $\ell>2$} \\
        &O(d \log{d} ) \qquad \text{if $\ell=2$} \\
        &O(d) \qquad \hspace{2.2em}\text{if $\ell=1$}.
    \end{cases}
\end{align}
These bounds have been improved by \cite{damian_2023_smoothing} up to order $d^{\ell/2}$; the latter matches the so-called \emph{Correlated Statistical Query} lower bound, which considers queries of the form $\Ea{y \phi(\vec{z})}$.

However, this Information Exponent is not the right measure of complexity for low-dimensional weak recovery. Indeed, \cite{damian2024computational} introduce a new Generative Exponent $\ell^\star$ (generative exponent) governing the weak recovery time scaling for algorithms in the Statistical Query (SQ) or Low Degree Polynomial (LDP) family. This exponent is defined as
\begin{equation}
    \ell^\star = \min \{ k \in \N \::\: \Eb{x \sim \cN(0, 1)}{f(h^\star(x))H_k(x)} \neq 0 \ \text{for some} \ f: \R \to \R \},
\end{equation}
which allows for the application of arbitrary transformations of the labels before performing the queries. Under this definition, the ``hard'' problems with $\ell^\star > 2$ are also impossible to learn for the best first-order algorithm, \emph{Approximate Message Passing} \citep{barbier2019optimal,celentano2021highdimensional,mondelli2018fundamental,luo2019optimal,maillard2020phase}.

We discuss in this work the extension of the generative exponent to the multi-index setting and investigate the dynamics of specific gradient-based programs (Algorithm~\ref{algo:optimizer_main_step}) as a function of the freshly defined hardness exponent $\ell^*$. 
These theoretical findings match the recent one of \cite{kou2024matching} on the computational efficiency of SGD in learning sparse $k-$parity (associated with $\ell^\star = k$).

When the optimal transformation $f$ is known, a simple SGD algorithm on $(\vec{z}, f(y))$ achieves the Generative Exponent lower bound. However, one problem remains: does there exist a class of SGD-like algorithms that can achieve this lower bound agnostically?

\paragraph{Achieving lower bounds with data repetition --}

Although the performance of single-pass SGD is limited by the Information Exponent of $h^\star$, the situation drastically changes when multiple-pass algorithms are considered. Recently, \cite{dandi2024benefits} proved that non-even single-index targets are weakly recovered in $T = O(d)$ when considering extensive batch sizes with multiple pass. This begs the question of how good can a ``reusing'' algorithm be. We answer this question for the class of polynomial link functions:
\begin{theorem}[Informal]
    There is a choice of hyperparameters such that if $h^\star$ is a polynomial function, Algorithm~\ref{algo:optimizer_main_step} achieves weak recovery in $O(d\log(d)^2)$ samples.
\end{theorem}
This shows that a simple gradient-based algorithm, which only requires seeing the data twice, is optimal for learning any polynomials.

\paragraph{Learning representations --}
The ability of learning relevant features/representations in the data is arguably one of the key properties of neural networks. However, a considerable attention in the theoretical community has been devoted to understanding the lazy training of two-layer networks \citep{jacot2018neural} where features are not effectively learned. Indeed, in this regime, shallow networks are equivalent to kernel machines, a class of fixed feature methods which are not able to adapt efficiently to low-dimensional relevant structure in the data (see e.g. \cite{Ghorbani2020}). Thus, understanding how representations are learned and providing corrections to the kernel regime is a central question in machine learning theory and has been explored in a variety of works (see e.g., \cite{pmlr-v75-dudeja18a, atanasov2022neural, Bietti2022, damian2022neural, petrini2022learning}). In this manuscript we provably characterize the number of iterations needed from Algorithm~\ref{algo:optimizer_main_step} to learn the relevant features of the data, i.e., attain weak recovery of the target subspace. Our results provide the scaling of the relevant hyperparameters $(\gamma, \rho)$ with the diverging input dimension $d$. The minibatch size will be fixed to $n_b =1$ in the main body, and we refer to Appendix~\ref{sec:app:numerics} for the extension to larger batch sizes.



\subsection*{Summary of Main Results}
\begin{itemize}
    \item \textcolor{purple}{Make explicit what is proven and what is not proven.}
    \item We prove for single-index targets that one-pass gradient-based algorithms are able to surpass the Correlation Statistical Query (CSQ) limitations established by the Information Exponent \citep{BenArous2021}.  
    \item We unveil that the dynamics of the family of Algorithm~\ref{algo:optimizer_main_step} are governed by the generative exponent introduced in \cite{damian2024computational} with an additional polynomial restriction on the transformation of the output.
    \item We generalize the notion of generative exponent to multi-index targets. Similarly to the single-index case, one-pass gradient-based algorithms can overcome CSQ performance dictated by the Leap Coefficient \citep{abbe2022merged}. 
    \item We prove that all polynomial multi-index functions are learned by Algorithm~\ref{algo:optimizer_main_step} either with total sample complexity $O(d)$ or $O(d \log(d)^2)$ if associated with the presence of a symmetry. 
    \item  The implementation of Algorithm~\ref{algo:optimizer_main_step} does not require pre-processing to initially correlate the estimation with the ground truth, and learns the meaningful representations from data alone. This is in contrast numerous findings (e.g., \cite{mondelli2018fundamental, luo2019optimal, maillard2020phase} for single index targets or \cite{chen2020learning} for multi-index ones).
    \item We characterize the class of hard functions not learned  in (almost) linear sample complexity. We show, however, that such functions can be learned through an hierarchical mechanism that extends the CSQ staircase first developed in \cite{abbe2021staircase} to a different, larger set, of functions.
    \item We validate the formal theoretical claims with detailed numerical illustrations. The code to reproduce representative figures is available in the Github repository \href{https://github.com/IdePHICS/Repetita-Iuvant}{https://github.com/IdePHICS/Repetita-Iuvant}.
\end{itemize}

==> sections_old/single_index.tex <==
\section{Single-Index Model}
\subsection{Main results}
We first consider, for simplicity, the class of single-index models, in which $k \!=\! p \!=\! 1$. This corresponds to a mismatched setting of Generalized Linear Models, in which we want to learn
\[ y = h^\star(\langle \vec{w^\star}, \vec{z} \rangle), \quad \text{with} \quad f(\vec{z}, \vec{w}, a) = a\sigma(\langle \vec{w}, \vec{z} \rangle). \]
In this section we rigorously characterize the number of iterations needed for the class of Algorithms~\ref{algo:optimizer_main_step} to perform weak recovery (as in Definition~\ref{def:weak_recovery}) in the context of single-index targets. We establish a clear separation between the the learning efficiency of the algorithmic  family~\ref{algo:optimizer_main_step} and One-Pass SGD, limited by the Information Exponent of the target to be learned \citep{BenArous2021}.

We start by introducing a restriction of the generative information exponent in \cite{damian2024computational} to polynomial transformations.
\begin{definition}[Polynomial Generative Information exponent]
\label{def:lstar_damian2024}
We define $\ell^\star_p$ as the smallest integer $k$ such that there exists a polynomial $p: \R \rightarrow \R$ with:
\begin{equation}\label{eq:f_hard_gen}
        \Eb{x\sim\cN(0, 1)}{p(h^\star(x))H_{k}(x)}\neq 0,
    \end{equation}
\end{definition}

Our assumptions on the SGD implementation and the target function are as follows:
\begin{assumption}\label{assump:spherical_corr}
    Algorithm \ref{algo:optimizer_main_step} is run with single-sample steps ($n_b = 1$), and uses the correlation loss
    \[ \cL(y, \hat y) = 1 - y\hat y.\]
    We also consider a spherical version of Alg. \ref{algo:optimizer_main_step}, with
    \begin{equation}\label{eq:spherical_sam}
        \vec{w}_{t+1} = \frac{\vec w_{t} - \gamma\nabla^\bot_{\vec w}
     \cL
    \left(
    f (\vec z^\nu; 
    \tilde{\vec{w}}_t(\rho), a_0),  y^\nu  \right)}{\norm{\vec w_{t} - \gamma\nabla^\bot_{\vec w}
     \cL
    \left(
    f (\vec z^\nu; 
    \tilde{\vec{w}}_t(\rho), a_0),  y^\nu  \right)}}
    \end{equation}
    where $\nabla^\bot f = \nabla f - \langle \nabla f, \vec{w} \rangle \vec{w}$ is the spherical gradient.
\end{assumption}

\begin{assumption}\label{assump:derivatives}
    The activation $\sigma$ is analytic almost everywhere, and $\sigma^{(n)}$ satisfies the polynomial growth assumption \eqref{eq:poly_growth} for $n \in \mathbb{N}$ (possibly for different constants $C_n$). Further, for all $n \geq 1$, we have
    \[ \Eb{x\sim\cN(0, 1)}{\sigma^{(n)}(x) \sigma'(x)^{n-1}} \neq 0 \quad \text{and} \quad \Eb{x\sim\cN(0, 1)}{x \sigma^{(n)}(x) \sigma'(x)^{n-1}} \neq 0 \]
\end{assumption}

\begin{assumption}\label{assump:init}
For a sign $\epsilon \in\{\pm 1\}$ depending on $h^\star$ and $\sigma$:
\begin{itemize}
    \item if $\ell_p^\star = 1$, $a_0 \neq 0$ the initial value $\vec{w}_0$ is drawn according to the uniform measure on
    \[ \mathbb{S}_\epsilon = \{ \vec{w}\in\mathbb{S}^{d-1} :\: \mathrm{sign}(\langle \vec{w}, \vec{w^\star} \rangle) = \epsilon \} \]
    \item if $\ell_p^\star = 2$, $\vec{w}_0$ is drawn uniformly in $\mathbb{S}^{d-1}$, and $a_0$ is such that $\operatorname{sign}(a_0) = \epsilon$.
\end{itemize}
\end{assumption}

We are now ready to state our main result.
\begin{theorem}
\label{thm:single_index_recovery}
    Suppose that Assumptions \ref{assump:poly_growth}-\ref{assump:init} hold, and let $\rho = \rho_0 d^{-1}$. Then, for any $\delta > 0$, there exists constants $\gamma_0(\delta)$ and $C(\delta)$ such that the following holds:
    \begin{itemize}
        \item If $\ell_p^\star = 1$, choosing $\gamma = \gamma_0(\delta)d^{-1}$, then
$
             \dP(t^+_\eta \leq C(\delta) \cdot d) \geq 1 - \delta
     $,

        \item If $\ell_p^\star = 2$, choosing $\gamma = \gamma_0(\delta)[d\log(d)]^{-1}$, then 
        $
            \dP(t^+_\eta \leq C(\delta) \cdot d \log(d)^2) \geq 1 - \delta
       $.
    \end{itemize}
    The above holds for almost every choice of $\rho_0$ under the Lebesgue measure.
\end{theorem}

\paragraph {Proof Sketch --} We provide here the proof sketch for Theorem~\ref{thm:single_index_recovery}. For any vector $\vec{w}$, under the correlation loss, we have
\begin{equation}\label{eq:sgd_gradient}
    \nabla_{\vec{w}} \cL(f(\vec{z}; \vec{w}, a_0), y) = a_0 y \sigma'(\langle \vec{w}, z \rangle) \cdot \vec{z},
\end{equation}
so the gradient is aligned with $\vec{z}$. As a result, we have
\begin{equation}\label{eq:sam_gradient}
    \nabla_{\vec w}\cL\left(f(\vec z; \tilde{\vec{w}}(\rho), a_0),  y \right) = a_0 y \sigma'\big(\langle \vec{w}, \vec{z} \rangle + a_0 \rho y \sigma'(\langle \vec{w}, \vec{z} \rangle) \cdot \underbrace{\norm{\vec{z}}^2}_{\approx d}\big) \cdot \vec{z}
\end{equation}
This expression for the gradient exhibits two important properties:
\begin{itemize}[itemsep=1pt,leftmargin=1em]
    \item Even though $\rho \asymp d^{-1}$, since the gradient lies along $\vec{z}$, the additional dot product with $\vec{z}$ amplifies the signal by a factor of $d$,
    \item The resulting gradient  \eqref{eq:sam_gradient} is a \emph{non-linear} function of $y$, as opposed to the linear function of \eqref{eq:sgd_gradient}. 
\end{itemize}
The latter property enables us to show that the dynamics driven by equation \eqref{eq:sam_gradient} can implement all polynomial transformations of the output $y$, for almost all choices of $\rho_0$. Subsequently, the SGD algorithm on the transformed input $p(y)$ can be studied with the same techniques as \cite{BenArous2021}, but with an information exponent equal to $\ell_p^\star$.

\subsection{Discussion}

\paragraph{Significance and necessity of the assumptions --}
Assumption \ref{assump:spherical_corr} simplifies Alg. \ref{algo:optimizer_main_step} to a more tractable version. In particular, the normalization step allows us to keep track of only one parameter, the overlap between $\vec{w}_t$ and $\vec{w}^\star$. We expect however Thm.\ref{thm:single_index_recovery} to hold in the general setting of Alg.\ref{algo:optimizer_main_step}.

Assumption \ref{assump:derivatives} is a regularity assumption, ensuring that some quantities of interest in the proof are non-zero. The first part is satisfied by virtually every activation function; the second is more restrictive, but we show that it is satisfied for biased activations:
\begin{lemma}\label{lem:bias_activation}
    Let $\sigma$ be a non-polynomial analytic function. Then the second part of Assumption \ref{assump:derivatives} is true for the function $x \mapsto \sigma(x + b)$ for almost every choice of $b$ (according to the Lebesgue measure).
\end{lemma}

Assumption \ref{assump:init} is similar to the one in \cite{BenArous2021}, and is necessary to ensure that the gradient at initialization does not point towards zero overlap, either because of a saddle or a local minimum. For random initialization of $\vec{w}$ and $a_0$, this assumption is satisfied with probability $1/2$.

Finally, although we state our result as an almost sure event over $\rho_0$, it can be reformulated into an event on the second layer weight $a_0$, in which the randomness comes from the initialization step.


\paragraph {Learning polynomial functions --} Although our definition of the Polynomial Generative Information exponent is more restrictive than the one in \cite{damian2024computational}, we show that it is enough to allow learning of a large class of functions, namely polynomials:
\begin{theorem}\label{thm:poly_pge}
    Assume that $h^\star$ is a polynomial function. Then the Polynomial Generative Information exponent of $h^\star$ is always at most 2, and is equal to 1 whenever $h^\star$ is not even.
\end{theorem}
This theorem implies that the Extragradient algorithm class allows us to match the sample complexity of the algorithm of \cite{chen2020learning}, without the need for \emph{ad hoc} preprocessing.

\paragraph{Beyond Algorithm~\ref{algo:optimizer_main_step} --} A succinct summary of the proof goes as follows: the first time we see a sample $\vec{z}$, we store information about $y$ along the direction of $\vec{z}$. The second time we see the same sample, the component along $\vec{z}$ in $\vec{w}$ interact \emph{non-linearly} with $y$, which bypasses the CSQ framework. Importantly, we expect that this behavior also appears in SGD algorithms where we do not see the data twice \emph{in a row}, but \emph{across multiple epochs}! Indeed, upon small enough correlation between the $\vec{z}^\nu$, seeing multiple examples before the repetition of $\vec{z}$ should not interfere with the data stored along this direction.
We are therefore not claiming that Algorithm~\ref{algo:optimizer_main_step} is superior to other classically-used methods; rather, it provides a tractable and realistic setting to study data repetition in SGD, which was ignored in previous theoretical works on the topic. 

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[height=0.95\textwidth, trim={0 8 0 0}, clip]{figures/fig1_ReluRelu.pdf}
        \caption{$h^\star(x) = \operatorname{relu}(x)$}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[height=0.95\textwidth, trim={0 8 0 0}, clip]{figures/fig1_H2Relu.pdf}
        \caption{$h^\star(x) = \mathrm{He}_2(x)$}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[height=0.95\textwidth, trim={0 8 0 0}, clip]{figures/fig1_H3Relu.pdf}
        \caption{$h^\star(x) = \mathrm{He}_3(x)$}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[height=0.95\textwidth, trim={0 8 0 0}, clip]{figures/fig1_H4Relu.pdf}
        \caption{$h^\star(x) = \mathrm{He}_4(x)$}
    \end{subfigure}
    \caption{\textbf{Learning single-index targets --}
    Evolution of the Cosine Similarity attained by EgD (crosses) and SGD (dots) as a function of normalized iteration time.
    The dashed horizontal line $\frac{1}{\sqrt{d}}$ is a visual guide to place random performance.
    \textbf{(a) $(\ell,\ell^\star)=(1,1)$:} both the algorithm learn in linear time.
    \textbf{(b) $(\ell,\ell^\star)=(2,2)$:} both the algorithm learn in \(O(d\log d)\) time.
    \textbf{(c) $(\ell,\ell^\star)=(3,1)$:} EgD learns in linear time, while SGD would learn the same function in quadratic time.
    \textbf{(d) $(\ell,\ell^\star)=(4,2)$:} EgD learns in \(O(d\log d)\) time, while SGD would learn in \(O(d^3)\) time.
    See all the details in App.~\ref{sec:app:implementation}.}
    \label{fig:main:single_index_complete}
\end{figure}

\subsection{Numerical illustrations}\label{subsec:single_numerics}
We illustrate in Fig.~\ref{fig:main:single_index_complete} the stark difference between the weak recovery dynamics of One-Pass SGD and Algo.~\ref{algo:optimizer_main_step} for single-index targets. The Cosine Similarity between the learned weight $\vec w_t$ and the ground truth informative direction $\vec w_\star$ is shown as a function of the time steps $t$ for different target functions. Two optimization routines are considered to exemplify the learning behaviour: a) Extragradient Descent (EgD), corresponding to the family of Algorithms~\ref{algo:optimizer_main_step} with positive $\rho$ parameters; b) One-Pass SGD, corresponding to vanilla SGD, or equivalently Algorithm~\ref{algo:optimizer_main_step} associated with $\rho=0$ hyperparameter. The scaling of $(\gamma, \rho)$ as a function of the input dimension  $d$ and exponent $\ell^\star$ are given in Thm.~\ref{thm:single_index_recovery}, while the mini-batch size is fixed to $n_b =1$ (See App.~\ref{sec:app:numerics} for extension to larger $n_b$). For all plots, we take $\sigma$ to be the $\mathrm{relu}$ activation and the implementation details can be found in Appendix \ref{sec:app:implementation}.

\textbf{SGD-easy non-symmetric targets ($\ell = \ell^\star =1$) --} The Left section of Fig.~\ref{fig:main:single_index_complete} shows $h^\star(x) = \mathrm{relu}(x)$. Here both SGD and Algorithm~\ref{algo:optimizer_main_step} learn in $T= O(d)$.
    
\textbf{SGD-easy symmetric targets ($\ell = \ell^\star = 2$) -- } The Center-Left section of Fig.~\ref{fig:main:single_index_complete} shows $ h^\star(x) = \mathrm{He}_2(x)$. Here both SGD and Algorithm~\ref{algo:optimizer_main_step} learn in $T=O(d \log d)$. 

\textbf{SGD-hard non-symmetric targets ($\ell > 2, \ell^\star =1$) -- }  The Center-Right section of Fig.~\ref{fig:main:single_index_complete} shows $ h^\star(x) = \mathrm{He}_3(x)$. Here Algortihm~\ref{algo:optimizer_main_step} learns in $T=O(d)$ while One Pass SGD suffers from the limitations detailed in eq.~\eqref{eq:gba_time_scaling}, i.e. $T= O(d^{\ell-1})$ with $\ell=3$ for this case.

\textbf{SGD-hard symmetric targets ($\ell > 2, \ell^\star =2$) -- } The Right section of Fig.~\ref{fig:main:single_index_complete} shows $h^\star(x) = \mathrm{He}_4(x)$. Here Algortihm~\ref{algo:optimizer_main_step} learns in $T=O(d \log d)$ while One Pass SGD suffers from the time scaling law detailed in eq.~\eqref{eq:gba_time_scaling} $T= O(d^{\ell-1})$.
